Development of recommendation systems for software engineering: the CROSSMINER experience

To perform their daily tasks, developers intensively make use of existing resources by consulting open-source software (OSS) repositories. Such platforms contain rich data sources, e.g., code snippets, documentation, and user discussions, that can be useful for supporting development activities. Over the last decades, several techniques and tools have been promoted to provide developers with innovative features, aiming to bring in improvements in terms of development effort, cost savings, and productivity. In the context of the EU H2020 CROSSMINER project, a set of recommendation systems has been conceived to assist software programmers in different phases of the development process. The systems provide developers with various artifacts, such as third-party libraries, documentation about how to use the APIs being adopted, or relevant API function calls. To develop such recommendations, various technical choices have been made to overcome issues related to several aspects including the lack of baselines, limited data availability, decisions about the performance measures, and evaluation approaches. This paper is an experience report to present the knowledge pertinent to the set of recommendation systems developed through the CROSSMINER project. We explain in detail the challenges we had to deal with, together with the related lessons learned when developing and evaluating these systems. Our aim is to provide the research community with concrete takeaway messages that are expected to be useful for those who want to develop or customize their own recommendation systems. The reported experiences can facilitate interesting discussions and research work, which in the end contribute to the advancement of recommendation systems applied to solve different issues in Software Engineering.

==> src/Context.tex <==
%Here we motivate and present CROSSMINER and the main objectives related to the need for RecSyc. Thus, the main challenges underpinning the need for recsys are discussed.


%\nb{Davide}{Discuss here the motivation behind CROSSMINER, i.e., 
%development of 
%new systems by relying on existing open source components}


\subsection{Source-code search}

Sourcerer\cite{linstead_sourcerer:_2009} is proposed aiming to 
perform code 
search in the large-scale repositories. The first component involved 
in the 
processing is the crawler, that downloads automatically the 
repositories. Then, 
the tool analyzes the code involving \emph{(i)} a parsing phase that 
maps each 
repository to the entity and possible relationships inserted in a 
relational 
database \emph{(ii)} Lucene module, that indexes the entities using 
keywords 
included in the code and \emph{(iii)} the ranker, that employs a 
graph-based 
representation of the code to filter and retrieve top rank results.
Beside this keyword-based technique, Sourcerer uses also the 
fingerprints, that 
summarize the snippets in vectors and give information about the 
syntactical 
information of the code. The tool uses them as support for structural 
search. 
Additionally, it search for best common practices in the computer 
science 
community i.e the most used name convention, analyzing the test 
classes, and 
the number of LOC. Then, it maps also the authors of each snippet 
using a 
matrix with author-document entries. In this way, Sourcerer can 
categorize the 
authors with the best skills according to their contributions. To 
evaluate the 
overall approach, the authors set up a user study on a dataset 
composed of over 
4,000 Java projects. They select 25 queries and do a manual 
evaluation on the 
results, involving also three expert developers, considering four key 
aspects: 
the original content of the query and the topic of the search, the 
quality of 
the results in term of coverage, the reputation of the project and, 
the 
possible reuse as a software component. Beside the human evaluation, 
they also 
use classical recall and precision metrics to assess the quality of 
the 
results. According to these, Sourcerer achieves high precision and 
accuracy 
considering the queries previously selected. 

In this work \cite{DBLP:conf/sigir/Henningen91}, the author proposes 
a tool, 
called CodeFinder, that performs recommendations using the 
example-based 
programming technique. As claimed in the paper, the most difficult 
part is to 
build the query and understand what the developer really needs. A 
system that 
relies only on a keyword-based system doesn't provide good enough 
results, 
because it excludes results that should be interesting for the user's 
purpose. 
Another problem strongly related to the example-based technique is 
that the 
suggested code doesn't fit exactly on the user's needs. To solve 
these issues, 
CodeFinder implements a hybrid approach that mixes the keyword-based 
style with 
information retrieval techniques, like the retrieval by reformulation 
that 
considers a subset of a concept instead try to match the exact one. 
To do this, 
the tool builds a network, that represents the conceptual model of 
the user, in 
which the keywords are induced by the query that the user is writing, 
using 
also the thesaurus to find synonyms that are more closer with respect 
to the 
query.  In the network, the keywords are the nodes and the 
relationship between 
them represent the level of likelihood. Once the user performs the 
first time 
the query, the CodeFinder interface retrieves other related keywords, 
the 
matching items and some code example of them. At this point, the 
interface 
allows adding new keywords in order to improve the query, exploiting 
the 
retrieval by reformulation technique. The key idea of this work is to 
guess the 
overall intentions of the developer when she writes some code, 
instead to 
reasoning only on the code or the query. Unfortunately, the 
validation of the 
tool is not available, as claimed by the author in the paper.


Facoy \cite{kim_f_2018} is a code-to-code search engine that 
recommends relevant
GitHub code snippets to a project being developed. Facoy is based on 
alternate 
query technique to enlarge the set of possible retrieved code 
snippets. The aim 
is to find similar posts on SO considering the semantic and not only 
the 
syntactic structure of the snippet of code. To this end, Facoy uses 
Lucene to 
set indexes that represent the relationship between the code and the 
semantic. 
In particular, a \emph{snippet index} is created to associate the 
answer 
document IDs with the code in the SO posts. To excerpt relevant 
information, 
Facoy parses the AST of the code, by wrapping the incomplete code in 
a dummy 
class in case of not compilable code. The second index \ie 
\emph{question 
	index} maps the information between the question and the source 
	code in the SO 
posts. Both created indexes are used to perform semantic analysis 
needed to 
build alternate queries that should. As the final step, Facoy 
computes an 
additional index \ie the \emph{code index} to search the similarity 
between the 
developer's code and the SO post. A user study has been set up to 
evaluate the 
obtained results. The questionnaire is composed of four different 
research 
questions aiming to measure  precision and accuracy of Facoy against 
the other 
code search engines. The used dataset considers 10.449 Github 
projects and the 
SO dump from 2008 to 2016. The user study shows that Facoy 
outperforms Krugle 
and Searchcode, the two code search engine considered in the 
comparison. 


\subsection{Source code recommenders}

Strathcona~\cite{holmes_strathcona_nodate} is a recommendation tool, 
which 
analyzes developer's context from the structural point of 
view and suggests a possible implementation related to the task that 
she is 
developing. Strathcona uses six heuristics based on 
inheritance hierarchy, field types method calls, and object usage in 
order to 
build the query. The built query is then executed on a repository 
containing 
all possible usage of the APIs and it is built automatically from the 
context. 
Finally, Strathcona retrieves code examples, which can be navigated 
by the 
developer both graphically and in a textual way.  

In \cite{DBLP:conf/aics/ZhengPL18} the authors propose Codex to 
detect 
plagiarism in the source code by exploiting similarity analysis based 
on 
fingerprints. It summarizes the AST of the code and then generates 
the 
respective fingerprint to represent relevant information of the tree. 
In 
particular, Codex gives a specific weight to each fingerprint using a 
fine-grained analysis. This mechanism assigns a lower score to 
so-called tiny 
terms  \ie parameters or constant that have less impact than bigger 
nodes in 
the tree. Codex analyze also the occurrence of sibling functions and 
compare 
the fingerprints of the subtrees following the top-down order. Once 
these 
weights are computed, the tool performs the search considering two 
levels of 
similarity. The local similarity compares the pair the developer's 
context with 
a single snippet. Reversely, the global similarity is obtained by 
comparing the 
fingerprint of the developer's code with the whole corpus. To this 
end, the 
tool walks the ASTs and prunes unnecessary nodes  according to a 
given 
threshold. To assess the quality of Codex, the evaluation is run over 
a dataset 
of 10 test cases with plagiarized code, 5 written in Python and 5 in 
Java. The 
dataset has different kinds of plagiarism, such as code modification, 
comments 
insertion, block combination. The results show that proposed tool is 
able to 
recognize the duplicated code in almost test cases, with accuracy 
near to 90\%.


In this work \cite{luan_aroma:_2018}, the authors propose Aroma, a 
tool that 
integrates code recommendations directly on the developer's context 
by 
employing a custom clustering technique. The first step is a 
light-weight 
search involving a simplified parse tree of the code. From this 
format, the 
tool is able to extract are the following features:

\begin{itemize}
	\item Token feature: it describes the token itself and they 
	consider only 
	local variable in the comparison, as the global ones are not 
	involved in 
	the alpha renaming process;
	\item Parent feature: this feature summarizes the structural 
	information of 
	the snippet;
	\item Sibling feature: it considers the previous and next element 
	of the 
	actual token;
	\item Variable usage feature: it represents the context in which 
	the token 
	is used and it is used to approximate the usage of the same local 
	variable
\end{itemize}

The light-weight search involves a list of methods body that overlaps 
the query 
body. A simplified parse tree is created to represent valuable 
information 
about the pair. Then, Aroma maps the information of the source code 
into a 
methods-features matrix to calculate the overlap score  . 
Additionally, a 
containment score is defined by applying a modified version of 
Jaccard distance 
on the quadratic time greedy algorithm. This score is employed to 
refine the 
results obtained with the overlap score.
By pruning recursively the results, Aroma obtains the list of tokens 
that reach 
the higher containment score. Finally, the tool creates clusters and 
their 
intersections using the obtained results in the previous phase. A 
commonality 
score is defined to guarantee a higher similarity among clusters. 
Aroma uses 
the computed clusters to excerpt representative tuples of simplified 
parse 
trees. Final recommendations are retrieved by intersecting each 
element of the 
clusters to find the most representative one. To assess the quality 
of the 
work, different evaluation scenarios have been proposed to considers 
different 
types of code recommendations. In the first scenario, the dataset is 
composed 
of 64 code snippets coming from StackOverflow posts. Each snippet is 
divided 
one half in the first run and analyze all the query body in the 
second one. 
They also manually categorize each query to consider their semantic 
\ie if the 
snippet configures an object to be used, it belongs to Configuring 
object 
categories. The results show that Aroma is able to retrieve the exact 
code most 
of the time.

In the second evaluation scenario, they measure the recall related to 
the 
second phase of the process, namely the pruning. The authors want to 
emphasize 
these results because the pruning and reranking represent the major 
element of 
novelty of the work. This evaluation shows that Aroma overcomes both 
the 
standard search techniques, i.e. keyword-based and feature-based 
searches, and 
the code cloning analysis. Finally, as they come out with a plug-in 
version of 
Aroma, they conduct also a user study in which developers are called 
to 
implement two coding tasks using Aroma. The major of participants 
found Aroma 
useful for the proposed tasks. Moreover, Aroma supports 4 different 
programming 
language namely Java, Python, JavaScript, and Hack.


Getafix \cite{bader_getafix:_2019} a tool that automatically fixes 
bug issues 
in the code. It includes the learning phase, in which the underlined 
model is 
trained with human-written code, and the predicting phase, where 
Getafix is 
able to recognize and fix the code given as input. The overall 
approach is 
based on the anti-unification technique, used to generalize patterns 
and 
extract structural information from them. The first step involves the 
representation of the source code by means of custom annotated AST. 
Once 
Getafix obtains the trees, it computes the edit distance to detect 
differences 
between the two version of the code. The tree patterns are 
generalized by using 
anti-unification and then they are clusterized by using a custom 
technique. In 
this way, Getafix reduces the possible candidates to fix a particular 
bug and 
picks the most representative ones. To increase efficiency, the tool 
considers 
also the code and error context in the tree edit patterns. The first 
type of 
context is useful to apply the pattern to a new segment of code while 
the 
second context is used to tailor the fix according to the errors 
involved. 
Finally, Getafix ranks the results and retrieve possible fixes for 
each 
category of bug. It considers three different scores by involving 
also 
human-written code. The prevalence score is higher for the patterns 
that cover 
human snippets. The location score measures the impact of a pattern 
in a 
particular location of the source core. Finally, the specialization 
score is 
higher for patterns that cover a very specific situation. To perform 
the 
ranking, there three scores are combined to retrieve the most 
representative 
patterns given a certain bug. To evaluate the approach, the authors 
set up 
10-fold cross-validation by using a dataset of 1.268 pairs of after 
and before 
files. They select 6 different types of bug and measure the accuracy 
for each 
of them. The results show that Getafix overcomes in most of the cases 
against 
the other baselines. Moreover, they conduct a user evaluation in 
which 42\% of 
participants accept the solutions proposed by Getafix. 



\subsection{API documentation and Q\&A recommenders}

CodeHow \cite{lv_codehow:_2015} supports software development task  
by using 
API documentation and the Extended Boolean model. As the initial 
step, the tool 
retrieves and parser the information coming from the API online 
documentation 
using the classical text preprocessing techniques \ie text 
normalization, stop 
words removal and stemming. In this way, CodeHow is able to find 
similarities 
between the user’s query and the API related to it. Then, it uses the 
Apache 
Lucene library to index the results. The main contribution of the 
work is the 
Extended Boolean Model (EBM) that is able to retrieve relevant 
results. This 
model is a trade-off between the two  the classical Boolean model and 
the 
Vector Space Model (VSM) because it assigns weights that belongs to 
the [0,1] 
interval and then normalizes the metric using the p-value set to 3.
To assess the quality of the approach, the authors use a dataset 
composed of 
26.000 C\# projects. Considering this dataset, they perform first an 
internal 
experiment composed of 34 real queries coming from the literature and 
checking 
by hand the top 20 results for each query. In addition, they perform 
a user 
evaluation involving 20 Microsoft developers who are called to 
implement three 
different tasks: the first one regards the sending emails, the second 
concerns 
the conversion from text to XML and the last the image format 
conversion. The 
authors compare their approach with Ohloh, another code search 
engine. From 
this comparison, CodeHow outperforms the opponent considering MRR and 
precision 
metrics.

Prompter~\cite{ponzanelli_prompter:_2016}  
is an automatic tool which is used to recommend SO posts given an 
input 
context built from source code. The tool performs 
various processing steps to produce a query. First, 
it splits identifiers and removes stop words. Then 
it ranks the terms according to their frequency by 
considering also the entropy of the term in the 
entire SO dump. Once the query is built, the tool 
exploits a web service to perform the query 
via the Google and Bing search engines. Finally, a 
ranking model is employed to sort the results 
according to different metrics such as API 
similarity, tags analysis, and SO answers and 
questions. 





==> src/CrossRec.tex <==
Finding and reusing third-party libraries are activities that programmers 
regularly perform during the development phase. Third-party libraries are 
highly advantageous to the development activities since they provide 
programmers with several tailor-made functionalities \cite{7985674}. Instead of 
programming from scratch, one only needs to search for libraries that implement 
the desired functionalities and embed into the existing code 
\cite{robillard_recommendation_2014}. For instance, in many Android apps, 
third-party 
libraries are a staple element \cite{Ma:2016:LFA:2889160.2889178}, a recent 
study shows that sub-packages from external libraries account for $60\%$ of 
code in Android software \cite{Wang:2015:WSA:2771783.2771795}.
%
Nevertheless, due to the heterogeneity of resources and their corresponding 
dependencies, developers need to spend a lot of effort to search for relevant 
items \cite{robillard_recommendation_2014}. 

%Despite the necessity, very little 
%work has been conducted concerning the techniques that facilitate the search 
%for suitable libraries from OSS repositories. Most of the related studies 
%address the issue of finding code snippets 
%\cite{Thummalapenta:2007:PPA:1321631.1321663} or API function calls 
%\cite{Thung:2013:ARA:3107656.3107694}. LibRec \cite{6671293} is among the most 
%advanced techniques for library recommendation to support OSS developers. It 
%was designed to find relevant libraries, based on the current set of items 
%that 
%a project already includes. LibRec has been demonstrated to be able to 
%recommend project libraries with a high \emph{success rate}. However, as 
%shown  
%in \cite{Nguyen:2019:JSS:CrossRec}, the performance of the approach can be 
%improved with respect to different quality metrics. 

%This section covers the use case \textbf{GetRecommendedDocs} as depicted in Figure~\ref{fig:Recommendations}.

\CR~\cite{Nguyen:2019:JSS:CrossRec} is a framework that exploits {\bf C}ross Projects {\bf R}elationships 
among {\bf O}pen {\bf S}ource {\bf S}oftware Repositories to build a {\bf 
Rec}ommendation System. With regards to the rich metadata infrastructure available 
at OSS repositories, we represent the cross relationships among them by 
exploiting the 
graph model already used in \CS, so as to compute similarities among various 
artifacts. We propose 
a novel approach utilizing a collaborative-filtering technique 
\cite{Schafer:2007:CFR:1768197.1768208} to recommend third-party libraries to 
support OSS developers. Originally, the technique was developed for e-commerce 
systems to exploit the relationships among users and products to predict the 
missing ratings of prospective items 
\cite{Linden:2003:ARI:642462.642471,Ouni:2017:SSL:3032135.3032325}. The 
technique is based on the premise that \emph{``if users agree about the quality 
or relevance of some items, then they will likely agree about other items''} 
\cite{Schafer:2007:CFR:1768197.1768208}. Our approach is derived from this to 
solve the problem of library recommendation. Instead of recommending goods or 
services to customers, we recommend third-party libraries to projects using an 
analogous mechanism: \emph{``if projects share some libraries in common, then 
they will probably share other common libraries.''} In other words, we work 
towards the search for an appropriate answer for the question: \emph{``Which 
third-party libraries should I further include in my current project?''} Thus, 
\CR supports software developers who have already included some 
libraries in the new projects being developed, and expect to get 
recommendations on which additional libraries should be further incorporated 
(if any). 
%
%
%
%To this end, the main contributions of this chapter are as follows: %is 
%%organized in the following sections: %in this paper 
%
%\begin{itemize}
%	\item Introducing a representation model to describe the relationship among 
%projects and third-party libraries in OSS repositories and to compute 
%similarities;	
%	\item Building a collaborative-filtering recommender system to assist 
%software developers with the selection of suitable third-party libraries; 
%%%\textbf{[??Add something more about collaborative-filtering (from LibFinder 
%%paper)]}
%	\item Proposing a set of metrics for the measurement of quality of 
%suggestions provided by a library recommender system. Besides \emph{success 
%rate}, we consider also \emph{accuracy}, \emph{sales diversity}, 
%\emph{novelty} 
%as they have been widely utilized in evaluating recommender systems 
%\cite{Nguyen:2015:CRV:2942298.2942305},\cite{robillard_recommendation_2014};
%	\item Performing an empirical study on the performance of \CR and 
%LibRec with a dataset of $1.200$ GitHub Java projects utilizing the above 
%mentioned quality metrics.
%\end{itemize}
%

The architecture of \CR is shown in Fig.~\ref{fig:CrossRecArchitecture} 
and it consists of the software components supporting the following activities:

\begin{itemize}
	\item \textit{Representing the relationships} among projects and libraries 
	retrieved from existing repositories;
	\item \textit{Computing similarities} to find projects, which are similar 
	to that under development;
	\item \textit{Recommending libraries} by using a 
	collaborative-filtering technique.
\end{itemize}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.68\textwidth]{figs/CrossRec.pdf}
	\caption{\CR's architecture \cite{Nguyen:2019:JSS:CrossRec}.}
	\label{fig:CrossRecArchitecture}
\end{figure}

In particular, as shown in Fig.~\ref{fig:CrossRecArchitecture}, the developer interacts with the system by sending a request for recommendations. The request contains a list of libraries that are already included in the current project. \emph{Data Encoder} collects background data from OSS repositories, represents them in a \emph{mathematically computable format}, which is then used as a base for other components of \CR. \emph{Similarity Computation} module calculates similarities among projects to find the most similar ones to the given project. \emph{Recommendation Engine} gets the list of \emph{top-k} similar projects and executes recommendation techniques to generate a ranked list of \emph{top-N} libraries. Finally, the recommendations are sent back to the developer. Background data can be collected from different OSS platforms like GitHub\footnote{GitHub \url{https://www.github.com}}, Eclipse\footnote{Eclipse \url{https://projects.eclipse.org}}, BitBucket.\footnote{BitBucket \url{https://www.bitbucket.com}}
The current version of \CR supports data extraction from GitHub, even though the support for additional platforms is already under development.


\emph{Recommendation Engine} works on the basis of an analogous 
user-item ratings matrix. To provide inputs for this module, the first task of 
\CR is to perform similarity computation to find the most similar 
projects to a given project. We adopted the \CS approach presented in the 
previous section as the mechanism 
for computing similarities among projects with respect to the included 
third-party libraries.

%\CR has been designed as a flexible framework and it can integrate 
%different similarity metrics as well as recommendation engines into its core. 
%The current implementation of \CR relies on \CS as the similarity 
%computation technique and the 
%user-based collaborative-filtering mechanism as the recommendation engine. 
%However, it is feasible to incorporate other similarity algorithms as well as 
%recommendation techniques as long as they are suitable to work on the metadata 
%available in OSS repositories.
%
%We conducted a comprehensive evaluation on LibRec and 
%\CR to see if and how well they are able to suggest suitable third-party 
%libraries. The approach has been evaluated by considering different quality 
%metrics and a dataset consisting of $1,200$ Java projects. The evaluation 
%demonstrated that 
%our approach outperforms LibRec, a well-known system for library 
%recommendation 
%with regards to various quality indicators. The CrossRec tool has been 
%successfully integrated into Eclipse and provided to developers as an IDE 
%prompting instant recommendations.



==> src/CrossSim2.tex <==
%GetProjectAlternativesWithSimilarAPIs


\CS~\cite{8498236,Nguyen:2019:JSS:CrossSim} is an approach for recommending similar projects with respect to the 
third-party library usage, given a specific project.
%Computing similarities among software systems is considered to be a difficult task 
%\cite{Chen:2015:SFD:2684822.2685305},\cite{McMillan:2012:DSS:2337223.2337267}.
%In addition, the miscellaneousness of artifacts in OSS repositories as well as 
%their cross relationship makes the similarity computation even more 
%complicated. For recommender systems in general, the ability to measure the 
%similarity between items plays an important role in obtaining relevant 
%recommendations \cite{Guo:2013:NBS:2540128.2540506}. Intuitively, for 
%software mining recommender systems, the measurement of similarities between 
%artifacts, e.g. projects, dependencies, code snippets, or even developers shall 
%also be a critical factor. Nevertheless, the computation of similarities 
%between software systems/open source projects in particular has been identified 
%as a thorny issue \cite{McMillan:2012:DSS:2337223.2337267}. Furthermore, 
%considering the miscellaneousness of artifacts in OSS repositories, similarity 
%computation becomes very complicated as many artifacts and several cross 
%relationships prevail.
%In OSS repositories, both humans, \ie developers and users or non-human actors, such as repositories, libraries have mutual dependency and implication on the others. The interactions among these components, such as developers commit to repositories, users star repositories, or projects include libraries, create a tie between them and should be included in similarity computation.
To enable both the representation of different OSS projects and the calculation of their similarity, a \textit{graph-based} model has been conceived. %Specifically, the model has been chosen since it allows for flexible data integration and facilitates numerous similarity metrics \cite{Blondel:2004:MSG:1035533.1035557}. 
We consider the community of developers together with OSS projects, libraries and all mutual interactions as an \textit{ecosystem}. Graphs are then used for representing different types of relationships in the OSS ecosystem.

As an example, we consider a set of four projects 
$P=\{p_1,p_2,p_3,p_4 \}$ and a set of libraries 
$L=\{$\emph{lib$_1$=junit:ju\-nit}; \emph{lib$_2$=commons-io:commons-io}; 
\emph{lib$_3$=log4j:log4j}; \emph{lib$_4$=org.slf4j:slf4j-api}; 
\emph{lib$_5$=org.slf4j:slf4j-log4j12}$\}$. By observing the \emph{pom.xml} 
files\footnote{The file \emph{pom.xml} defines all project dependencies with 
	external Maven libraries 
	(\url{https://maven.apache.org/guides/introduction/introduction-to-the-pom.html})
} of the projects in $P$, we discovered the following inclusions: $p_1 \ni 
lib_1,lib_2$; $p_2 \ni lib_1,lib_3$; $p_3 \ni lib_1,lib_3,lib_4,lib_5$; $p_4 
\ni lib_1,lib_2,lib_4,lib_5$. The graph for the set of projects is depicted in 
Fig.~\ref{fig:Graph}.

%According to \cite{McMillan:2012:DSS:2337223.2337267,6671293} the similarity between two considered projects relies on the dependencies they have in common because they aim at implementing similar functionalities.	

%As being inspired by the research from a related field, Linked Data and Semantic Web \cite{bizer_linked_2009}, we believe that a representation model that addresses the semantic relationships among miscellaneous factors in the OSS community should essentially beneficial to similarity computation. To this end, we consider the community of developers together with OSS projects, libraries and their mutual interactions as an \textit{ecosystem}. We derive a \textit{graph-based} model to represent different kinds of relationships in the OSS ecosystem and eventually to calculate similarities. Specifically, the graph model has been chosen since it allows for flexible data integration and numerous computation techniques \cite{Blondel:2004:MSG:1035533.1035557,Nguyen:2015:CRV:2942298.2942305,Nguyen:2015:ESP:2740908.2742141}. The graph structure also facilitates graph kernel methods, which are an effective way to compute similarities \cite{ODMD14a}. By applying this representation, we are able to transform the set of projects and libraries introduced in Section \ref{sec:Overview} into a directed graph as depicted in Figure \ref{fig:Graph}.


\begin{figure}[t!]
	\centering
	\includegraphics[width=0.60\textwidth]{figs/Graph.pdf}
	\caption{Graph representation for projects and libraries~\cite{8498236,Nguyen:2019:JSS:CrossSim}.} % [to be refined/changed]
	\label{fig:Graph}
\end{figure}


%In Linked Data, an RDF\footnote{RDF 1.1 Concepts and Abstract Syntax: \url{https://www.w3.org/TR/2014/REC-rdf11-concepts-20140225/}} graph is made up of an enormous number of nodes and oriented links with semantic relationships. Thanks to this feature, the similarity of two nodes in a graph can be computed by considering their intrinsic characteristics like neighbour nodes and their mutual interactions \cite{DiNoia:2012:LOD:2362499.2362501,Nguyen:2015:CRV:2942298.2942305}. 

We adopted an existing approach~\cite{DiNoia:2012:LOD:2362499.2362501} to compute the similarities among OSS 
graph nodes, as it has been successfully exploited by many studies to do the 
same task \cite{BRIGUEZ20146467}. Among other relationships, two nodes in a 
graph are deemed to be similar if they point to the same node with the same 
semantic edge. For instance, the graph in Fig.~\ref{fig:Graph} depicts the 
relationships among four projects and five third-party libraries. There, we see 
that $p_3$ and $p_4$ are highly similar since they both point to three nodes 
representing $lib_{1}, lib_{4}, lib_{5}$. This reflects the actual relationship 
of the two projects by the view of software engineering: they are similar since 
they implement common functionalities by using common libraries 
\cite{McMillan:2012:DSS:2337223.2337267}. By the view of recommendation 
algorithms, given a project $p$, suggested libraries for $p$ should come from 
the most similar projects to $p$ \cite{DBLP:conf/rweb/NoiaO15}.

%Since VsmSim quantifies similarities by using libraries per se, it is our firm belief that the technique will facilitate the search for similar projects with respect to dependency usage.
%in terms of
%By VsmSim\footnote{For the sake of clarity, the name is given by ourselves since the metric was not name by its authors}, 
%In this sense, it is highly important to find the most similar projects to $p$. Since  In this way,  Vector Space Model.  the nodes connected to it represented using a vector as follows
%Being based on the Vector Space Model  \cite{Turney:2010:FMV:1861751.1861756}, 
% with each entry corresponding to the weight or a neighbour node:


%
%Using this metric, the similarity between two project nodes $p$ and $q$ in an 
%OSS graph is computed by considering their feature sets 
%\cite{DiNoia:2012:LOD:2362499.2362501}. Given that $p$ has a set of neighbour 
%nodes $(lib_{1},lib_{2},..,lib_{n})$, the features of $p$ are represented by a 
%vector $\overrightarrow{\phi}=(\phi_{1},\phi_{2},..,\phi_{n})$, with 
%$\phi_{i}$ 
%being the weight of node $lib_{i}$. It is computed as the \emph{term-frequency 
%inverse document frequency} value as follows: %\texttt{tf-idf}   of the node 
%
%\begin{equation}\label{eqn:TFIDF}
%\phi_{i} = f_{lib_{i}}*log(\frac{ \left | P \right |}{a_{lib_{i}}})
%\end{equation}
%
%
%where $f_{lib_{i}}$ is the number of occurrence of $lib_{i}$ with respect to 
%$p$, it can be either $0$ and $1$ since there is a maximum of one $lib_{i}$ 
%connected to $p$ by the edge \emph{includes}; $\left | P \right |$ is the 
%number of projects in the collection; $a_{lib_{i}}$ is the number of projects 
%connecting to $lib_{i}$ via the edge \emph{includes}. According to 
%Eq.~\ref{eqn:TFIDF}, node $lib_{1}$ in Figure~\ref{fig:Graph} has a low weight 
%compared to other nodes since it is pointed by all four project nodes. In 
%practice, this is comprehensible since \emph{junit:junit} is a very popular 
%dependency and thus it should have a less important role in characterizing a 
%project.
%
%Eventually, the similarity between $p$ and $q$ with their corresponding 
%feature vectors $\overrightarrow{\phi}=\{\phi_{i}\}_{i=1,..,l}$ and 
%$\overrightarrow{\omega}=\{\omega_{j}\}_{j=1,..,m}$ is computed as given below:

%where $f_{l_{i}}$ is the number of occurrence of $l_{i}$ with respect to $p$, it can be either $0$ and $1$ since there is a maximum of one $l_{i}$ connected to $p$ by the edge \emph{includes}; $\left | P \right |$ is the number of projects in the collection; $a_{l_{i}}$ is the number of projects connecting to $l_{i}$ via the edge \emph{includes}. According to Equation \ref{eqn:TFIDF}, node $lib_{1}$ in Figure \ref{fig:Graph} has a low weight compared to that of other nodes since it is pointed by all four project nodes. In practice, this is comprehensible since \emph{junit:junit} is a very popular dependency and thus it should have a less important role in characterizing a project.
%Eventually, the similarity between $p$ and $q$ with their corresponding feature vectors $\overrightarrow{\phi}=\{\phi_{i}\}_{i=1,..,n}$ and $\overrightarrow{\omega}=\{\omega_{i}\}_{i=1,..,n}$ is computed as given below:

%
%\begin{equation} \label{eqn:VsmSim1}
%sim(p,q)=\frac{\sum_{i=1}^{n}\phi_{i}\times 
%\omega_{i}}{\sqrt{\sum_{i=1}^{n}(\phi_{i})^{2} }\times 
%\sqrt{\sum_{i=1}^{n}(\omega_{i})^{2}}} 
%\end{equation}

%where $n$ is the cardinality of the set of libraries that $p$ and $q$ share in 
%common \cite{DiNoia:2012:LOD:2362499.2362501}. Intuitively, $p$ and $q$ are 
%represented as vectors in an $n$-dimensional space and Eq.~\ref{eqn:VsmSim1} 
%measures the cosine of the angle between the two vectors. %and it is computed 
%%using the inner product as follows.





%the performance evaluation of this section into the one in. 
%as the Similarity Calculator




%\subsubsection{Get project alternative with similar size}





==> src/EvaluationMethodology.tex <==

%==================================================================================================================
%\subsection{Evaluation of CrossSim} \label{sec:CrossSimEvaluation}
%In addition, $RepoPal$ works on GitHub Java repositories containing rich metadata that is suitable for building graph in $CrossSim$. 
%To compare outcome with that of a ground-truth dataset. To evaluate the accuracy of the.
%Considering a 
%And we expect a list of results.%needs recommendations for third-party libraries. 
%==================================================================================================================
%To thoroughly study the performance of LibRec and CrossRec, 
%Our recommender system is able to generate various types of recommendations. To recommend a set of code snippets, or API usage patterns. with the presence of a dataset. 
% hereafter and numbered from $1$ to $10$, with each consisting of $120$ projects.
%cross validation is normally used, 
%We designed and implemented a collaborative-filtering system. The presence of training data and testing data. ground-truth data can be generated manually or automatically, depending on the domains. For example \cite{HaoranNiu}. Automatic: LibRec.

%When a fold is used as testing data, library recommendation will be conducted for all of its $120$ testing projects. For every testing project \emph{p}, a half of its libraries are taken out and saved as ground truth data, which will be used to validate the recommendation outcomes. The other half are used as testing libraries and serve as input for \code{Similarity Computation} and \code{Recommendation}. By each validation round, we use the same folds for testing and training by both recommender systems. Also for a testing project, the same sets of testing libraries and ground-truth libraries are used for experiments on LibRec and CrossRec. This is to make sure that the same condition is applied in both systems, so as to precisely validate their performance.
%It is validated using a ground-truth dataset. The metrics can be applied to evaluate different domains. To ease the presentation, in the scope of this paper, we consider a concrete example within the context of CROSSMINER as follows. A developer is working on a new software project and he has already included some third-party libraries. 
%The outcome of a recommendation process is a ranked list of items. 

%we applied ten-fold cross validation, which has been identified as among the best methods for model selection \cite{Kohavi:1995:SCB:1643031.1643047}. the dataset is divided into $10$ equal parts, named \emph{folds}.
%For each recommender system, the validation has been conducted in ten rounds. For each round $i$, the fold \emph{fold}$_i$ is used as \emph{testing data} and the remaining nine folds \emph{fold}$_j$ with $j \neq i, 1 \leq i,j \leq 10$ are used as \emph{training data} \cite{Cremonesi:2008:EMC:1468165.1468327}. The training data is used to compute similarity and serves as the background data for recommendation, while the testing data is used to validate the model \cite{arlot2010survey}.% \cite{Cremonesi:2008:EMC:1468165.1468327}.
%To study the outcomes, first we consider \emph{recall rate@N} which was used as the only evaluation metric for LibRec \cite{6671293}.
%There are the following evaluation metrics:
%Evaluation methodology. Using data, instead of.
%How to properly evaluate the outcome of a recommendation process. 
%in mining knowledge from OSS repositories

%For several studies in the domain of mining software repositories, performing a user study has been accepted as the standard method to validate an API usage recommendation tool \cite{Moreno:2015:IUT:2818754.2818860,10.1007/978-3-642-03013-0_15}. However, a user study is normally cumbersome and highly prone to individual perception. We introduce a validation approach that automatizes the evaluation by relying solely on data. Due to space limitation, we are able to introduce a preliminary evaluation on API function calls recommendation in this paper. We leave the evaluation of code snippets recommendation for our future work. We introduce an evaluation methodology that relies solely on data. 
%Moreno:2015:IUT:2818754.2818860,
% by existing studies
%as input of the recommendation process
%There are various methods of performing a validation. 
% \cite{Cremonesi:2008:EMC:1468165.1468327}
 
% \cite{Cremonesi:2008:EMC:1468165.1468327}
%==================================================================================================================

For recommender systems in mining OSS repositories, one of the key issues is 
how to properly evaluate their performance. Conducting a user study has been 
accepted as the \emph{de facto} way to analyze the outcome of a recommendation 
process by several studies 
\cite{McMillan:2012:DSS:2337223.2337267,Moreno:2015:IUT:2818754.2818860,Ponzanelli:2014:MST:2597073.2597077,10.1109/SANER.2017.7884605,10.1007/978-3-642-03013-0_15}.

\JDR{User study techniques generally interview the involved participants before and after the usage of a tool or an approach. In this respect, an experiment can include \textit{qualitative} and \textit{quantitative} analysis where the former involves descriptive and not measurable data, and the former involve information about measurable data, quantities, and therefore numbers. In the context of user evaluation the qualitative analysis is performed on informal conversation interview, guided interview and open-ended questions, whereas a quantitative analysis can be applied when an interview uses closed and fixed response (\ie the Likert scale which responses are scored among a range of agreement/disagreement).}

Nevertheless, a user study is, in general, labor intensive and prone to 
individual perception, which may introduce bias against the results.\JDR{We should include user evaluation techniques as an evaluation methodology} We believe 
that depending on the availability of data, we can avoid performing such a 
manual analysis. To this end, we propose an approach to evaluate the 
recommendation outcomes by relying solely on data.% in some specific cases,

Given a dataset used for evaluation, we split it into two independent parts, namely a \emph{training set} and a \emph{testing set}. In practice, the items in the training data correspond to the OSS projects that have been collected beforehand. They are available at developers' disposal, ready to be exploited for any mining purpose. Whereas, each item in the testing data represents the project being developed, or \emph{the active project}. The division of a dataset into training and testing data determines the validation method. Among others, \emph{k-fold cross validation} has been popularly chosen as the evaluation method for a model in Machine Learning. By this method, a dataset is divided into $k$ equal parts (\emph{folds}). For each validation round, one fold is used as testing data and the remaining \emph{k-1} folds are used as training data. In this sense, an evaluation attempts to mimic a real situation: \emph{the system should produce recommendations for a project based on the data available from a set of existing projects}. %Some possible values are $k=\{2,5,10\}$.}

We call the artifact being considered as the recommendation target as \emph{object}. For instance, regarding third-party libraries recommendation \cite{DBLP:conf/iir/NguyenRR18}, objects are libraries that a recommender system needs to provide as outcome. It is necessary to investigate if the recommender system can help by providing the active project with relevant objects, exploiting the training data. To this end, for each active project, we keep a certain amount of objects and use them as input for the recommendation engine, this can be understood as the query. The rest is taken out and used as \emph{ground-truth data}. Later on, the ground-truth data will be compared against the recommendation outcomes to validate the system's performance. Generally, it is expected that the recommender system can retrieve objects that match up the ones stored as ground-truth data.

By comparing the objects that are provided by the recommendation process with those stored as ground-truth data, we are able to investigate how well the recommender system performs.
\JDR{Similarly, in case we have limited data to training the recommendation system, one of the most used techniques is \emph{eave-one-out cross-validation}~\cite{WONG20152839} where one element of the dataset is used as testing element and the remaining ones are used as training data.}

\JDR{Several metrics have been involved to analyse the performance of recommendation systems. Next section lists the most used ones}. \JDR{Can we remove the following sentences? - There are several metrics which can be used to 
analyze the performance of a recommender system. To measure \emph{accuracy}, \emph{precision}, \emph{recall} are normally utilized \cite{DBLP:conf/iir/NguyenRR18}. However, accuracy is not sufficient for validating a recommender system's performance  \cite{Ge:2010:BAE:1864708.1864761}, other metrics should also be incorporated to analyze various quality aspects.
Among others, \emph{diversity}, \emph{novelty} are popular metrics for studying recommender systems. \emph{Diversity} means the ability of the system to suggest to projects as many items as possible, as well as to disperse the concentration among all the items. Whereas \emph{Novelty} measures if the system is able to expose items to the audience. Due to space limits, we refer the reader to our work in \cite{DBLP:conf/iir/NguyenRR18,FOCUS2019} for the preliminary results concerning the validation of recommendation results.}%\cite{Ge:2010_catalog_coverage}

\JDR{}

In summary, the presented methodolog\JDR{ies} can be applicable to evaluation of various recommendations. We anticipate that the scheme is suitable at least for the following types of recommendations: third-party libraries \cite{DBLP:conf/iir/NguyenRR18}, API usage patterns \cite{Moreno:2015:IUT:2818754.2818860,FOCUS2019}, and StackOverflow posts \cite{Ponzanelli:2014:MST:2597073.2597077}. %Additional evaluations may also be possible depending on the presence of input data. 



\CDS{We could divide this section into two main categories: automated evaluation and user evaluation.
For the former, I think the corresponding section is well-defined and it needs only some minor refinements. Concerning the user evaluation, we can indeed
show our experience gained in the past i.e., SOrec and CrossRec studies. Although they are not comprehensive approaches, I think we are able to give a flavor of our work and
the challenges that arise during this kind of activity (we can refer to these as "controlled studies" or something like that). We can mention also the difficulties to conduct more extensive studies i.e, we don't have enough people.***}

\vspace{-.3cm}

%It might be interesting if we can do something to show that novelty and diversity in the recommendation outcomes are meaningful. Currently, many existing approaches just choose to recommend popular items, \eg MUSE \cite{Moreno:2015:IUT:2818754.2818860}, PROMPTER \cite{Ponzanelli:2014:MST:2597073.2597077}, LibRec \cite{6671293}.

%, instead of focusing only on a specific set of them

%==================================================================================================================
%To see if a proposed model will perform well also in practice, we can simulate by using \emph{training data} and \emph{testing data}. User study, where the evaluation is done by involving humans. Depending on the availability of data, it is possible to automatize the evaluation process.
%The ground-truth data is used to validate the recommendation results. There are several metrics can be used to evaluate the performance of a recommender system, not only accuracy but other metrics should be considered, such as \emph{diversity}, \emph{novelty}. We refer the reader to the work presented in \cite{DBLP:conf/iir/NguyenRR18 } for a greater detail.  is background, it is already available, while testing data is.
% is among the most popular way to v.
%\subsection{Metrics}
%
%Given a query, the outcome of the recommendation process is a ranked list of items that are considered to be relevant for the query. For instance, a system that recommends third-party libraries for a given project returns a list in descending order of real similarity scores corresponding to libraries \cite{6671293}. To validate the performance of a recommender system, we need a \emph{training} and a \emph{testing} dataset \cite{Cremonesi:2008:EMC:1468165.1468327}. The former is used to build the model whereas the latter is used to validate the outcome. Considering a project that needs library recommendation, the graph model is used to compute similarities and then to find most $k$ similar projects. The outcome of the recommendation is a ranked list of third-party libraries. Normally, a developer pays attention only to the \emph{top-N} items. We use $k$ and $N$ as parameter for the evaluation later on.%for evaluation. %Afterwards, a 
%
%We recall the following metrics that can be used to evaluate the performance of a recommender system in the context of mining software repositories given the presence of training and testing datasets. First, for a clear presentation of the metrics considered during the outcome evaluation, the following notations are defined:
%
%
%\begin{itemize}
%	\item \emph{N} is the cut-off value for the list of recommended items and \emph{k} is the number of neighbour projects considered for the recommendation process;
%	\item For a testing project \emph{p}, the ground-truth dataset is named as \emph{GT(p)};	
%	\item $REC(p)$ is the \emph{top-N} items recommended to \emph{p}. It is a ranked list in descending order of real scores, with $REC_r(p)$ being the library in the position $r$;		
%	\item If a recommended item $i \in REC(p)$ for a testing project $p$ is found in the ground truth of $p$ (i.e., \emph{GT(p)}), hereafter we call this as a library \textit{match} or \textit{hit}.	
%\end{itemize}	
%
%
%Using these notations, the metrics utilized to measure the recommendation outcomes are explained in the following. Among others, we consider \emph{success rate} \cite{6671293}, \emph{accuracy} \cite{McMillan:2012:DSS:2337223.2337267}, \emph{sales diversity}, and \emph{novelty} the most suitable metrics for evaluating a recommender system in mining OSS repositories \cite{robillard_recommendation_2014}.% and they are recalled as follows.%, in the context of. 











==> src/EvaluationMetrics.tex <==
%\subsection{Evaluation of CrossSim} \label{sec:CrossSimEvaluation}
%In addition, $RepoPal$ works on GitHub Java repositories containing rich metadata that is suitable for building graph in $CrossSim$. 
%To compare outcome with that of a ground-truth dataset. To evaluate the accuracy of the.
%Considering a 
%And we expect a list of results.%needs recommendations for third-party libraries. 




%To thoroughly study the performance of LibRec and CrossRec, 
%Our recommender system is able to generate various types of recommendations. To recommend a set of code snippets, or API usage patterns. with the presence of a dataset. 
% hereafter and numbered from $1$ to $10$, with each consisting of $120$ projects.
%cross validation is normally used, 
%We designed and implemented a collaborative-filtering system. The presence of training data and testing data. ground-truth data can be generated manually or automatically, depending on the domains. For example \cite{HaoranNiu}. Automatic: LibRec.

%When a fold is used as testing data, library recommendation will be conducted for all of its $120$ testing projects. For every testing project \emph{p}, a half of its libraries are taken out and saved as ground truth data, which will be used to validate the recommendation outcomes. The other half are used as testing libraries and serve as input for \code{Similarity Computation} and \code{Recommendation}. By each validation round, we use the same folds for testing and training by both recommender systems. Also for a testing project, the same sets of testing libraries and ground-truth libraries are used for experiments on LibRec and CrossRec. This is to make sure that the same condition is applied in both systems, so as to precisely validate their performance.
%It is validated using a ground-truth dataset. The metrics can be applied to evaluate different domains. To ease the presentation, in the scope of this paper, we consider a concrete example within the context of CROSSMINER as follows. A developer is working on a new software project and he has already included some third-party libraries. 
%The outcome of a recommendation process is a ranked list of items. 

%we applied ten-fold cross validation, which has been identified as among the best methods for model selection \cite{Kohavi:1995:SCB:1643031.1643047}. the dataset is divided into $10$ equal parts, named \emph{folds}.
%For each recommender system, the validation has been conducted in ten rounds. For each round $i$, the fold \emph{fold}$_i$ is used as \emph{testing data} and the remaining nine folds \emph{fold}$_j$ with $j \neq i, 1 \leq i,j \leq 10$ are used as \emph{training data} \cite{Cremonesi:2008:EMC:1468165.1468327}. The training data is used to compute similarity and serves as the background data for recommendation, while the testing data is used to validate the model \cite{arlot2010survey}.% \cite{Cremonesi:2008:EMC:1468165.1468327}.
%To study the outcomes, first we consider \emph{recall rate@N} which was used as the only evaluation metric for LibRec \cite{6671293}.
%There are the following evaluation metrics:





==> src/FOCUS.tex <==
Third-party libraries are interface to runnable and reusable code snippets, 
they can be embedded in source code projects independently from environment 
code \cite{Robillard:2013:AAP:2498733.2498776}. For software developers, 
integrating external components into source code being developed is a daily 
routine since this helps accelerate the development process as well as increase 
reliability. Rather than programming from scratch, developers look for 
libraries that implement the desired functionalities and integrate them into 
their existing projects \cite{DBLP:conf/iir/NguyenRR18}. For such libraries, 
API 
function calls are the entry point which allows one to invoke the offered 
functionalities. However, in order to exploit a library to implement the 
required feature, programmers need to consult various sources, \eg API 
documentation to see how a specific API instance is utilized in the field. 
Nevertheless, from these external sources, there are only texts providing 
generic syntax or simple usage of the API, which may be less relevant to the 
current development context. In this sense, concrete examples of source code 
snippets that indicate how specific API function calls are deployed in actual 
usage, are of great use \cite{Moreno:2015:IUT:2818754.2818860}. %the. . 
%contain the API functions  (an insight)

With the \FC tool~\cite{Nguyen:2019:FRS:3339505.3339636} we assist developers in mining relevant API 
function calls and usage patterns from open source projects. The question that 
the tool is able to answer is: \textit{``Which API methods should this piece of 
client code invoke, considering that it has already invoked these other API 
methods?''} 

In particular, by a context-aware 
collaborative-filtering technique, given a customer who needs suggestions 
on what additional products should be put into the shopping cart, the intuition 
is to collaboratively deduce the presence of prospective items from \emph{those 
	that have been purchased by similar customers in comparable contexts} 
\cite{Chen:2005:CCF:2154509.2154540}. Here, similar customers and contexts play 
the role of a \emph{filter} that narrows down the search scope. To 
solve the problem of API usage recommendation, an analogous mechanism is applied: instead of 
searching in all projects, \FC looks for invocations only from 
similar projects, thus yielding the feature \emph{collaborative filtering}. By considering the following mappings: \emph{projects--contexts}, 
\emph{declarations--customers}, and \emph{invocations--products}, we are able 
to transform the model applied in products recommendation into a solution for 
recommending API usages. Intuitively, %as illustrated in Figure~\ref{fig:likening}, 
we simulate the situation when a customer (a 
declaration) wonders if she (it) should buy (incorporate) a product (an 
invocation) given a concrete context (the current project).
%
%%====================Here we introduce the problem of API function calls 
%%recommendation=============================================
%
%
%%==================================================================================================================================
%% 
%%StackOverflow \cite{Ponzanelli:2014:MST:2597073.2597077}
%
%%The first type is the recommendation of API call sequences where a developer 
%%is provided with a list of API functions. 
%%FOCUS recommends complete source code examples that are relevant to the 
%%method being developed, By the second type of recommendations, 
%%the developer herself needs to decide how to properly embed the functions
%%In this sense, identifying a set of API functions that are relevant to the 
%%current development context is of highly importance.
%%As already pointed out, such type of recommendations lacks of details of 
%%control flow and might be suitable only for skilled developers.
%%Clustering has been considered as the de factor mechanism for finding similar 
%%source code snippets 
%%\cite{10.1007/978-3-319-89363-1_11},\cite{10.1007/978-3-642-03013-0_15},\cite{6624045}.
%% Nevertheless, existing studies seem not to fully exploit the context data on 
%%which the developer is working to mine the most relevant API usages. In our 
%%view, the current project together with all API function calls, provide a 
%%precise insight into the development context and they should be properly 
%%incorporated into the recommendation process. 
%%==================================================================================================================================
%
%Two major types of API mining methods have been identified 
%\cite{10.1007/978-3-319-89363-1_11}. By the first type, a system suggests a 
%ranked list of API invocations and the programmer exercises her own discretion 
%in choosing suitable function calls. On one side, this scheme gives more 
%freedom to the integration process, on the other side, it lacks details of 
%control flow and might be suitable only for skilled developers. By the 
%second type of recommendations, the developer gets real code snippets that 
%implement specific functionalities and she can directly embed the most 
%relevant 
%snippet into the current function. Such recommendation is considered to be 
%more 
%practical and helpful. However, since an API function can be used in different 
%contexts depending on the purposes, simply recommending a code snippet that 
%contains some API functions may not be the solution, it can be irrelevant to 
%the context as a whole \cite{10.1007/978-3-642-03013-0_15}. 
%
%
%Clustering has been considered as the \textit{de facto} mechanism for finding 
%similar source code snippets, aiming to remove redundant items 
%\cite{10.1007/978-3-319-89363-1_11},\cite{10.1007/978-3-642-03013-0_15},\cite{6624045}.
%Nevertheless, a substantial amount of redundancy is still witnessed by 
%approaches that rely on clustering \cite{Fowkes:2016:PPA:2950290.2950319}. 
%Furthermore, existing studies seem not to fully exploit the context data on 
%which the developer is working to mine the most relevant API usages. In our 
%view, the current project together with all API function calls, provide a 
%precise insight into the development context and they should be properly 
%incorporated into the recommendation process. Within the scope of Work Package 
%$6$, we develop FOCUS, a context-aware collaborative filtering recommender 
%system that mines OSS repositories to provide developers with API 
%\textbf{F}uncti\textbf{O}n \textbf{C}alls and \textbf{US}age 
%patterns~\cite{Nguyen:2019:FRS:3339505.3339636}. FOCUS 
%concurrently supports two functionalities: API function calls recommendation 
%and API usage patterns recommendation.
%
%Our work distinguishes itself from other existing approaches in terms of the 
%following aspects. First, it employs a new model to represent the mutual 
%relationships in source code. Second, given a project, FOCUS collaboratively 
%mines API usage from the most similar projects. It attempts to narrow down the 
%search scope and to \emph{focus on} only the most relevant API usages by 
%\emph{collaboratively filtering out} irrelevant items. Furthermore, to the 
%best 
%of our knowledge, existing studies rely heavily on the manual analysis of 
%recommendation outcome by human to validate performance. Nonetheless, such an 
%analysis is labor intensive, time consuming and prone to subjective perception 
%\cite{Bruch:2008:ERS:1454247.1454254}. We get rid of a user study and 
%propose an approach to automate the evaluation process by means of cross 
%validation, splitting a dataset into independent subsets, namely 
%\emph{training 
%	data} and \emph{testing data}. In this sense, the main 
%contributions of this chapter are summarized as follows:
%
%%====================================================================================================================================================
%
%\begin{itemize}
%	\item Deploy a context-aware collaborative-filtering technique for 
%recommending API function calls and usage patterns;
%	\item Introduce an approach for evaluating the outcomes of API function 
%calls and usage patterns recommendation without relying on a user study;	
%	\item Evaluate the performance of the proposed approach on a dataset 
%curated from the Maven 
%repository\footnote{\href{https://mvnrepository.com}{https://mvnrepository.com}}.
%\end{itemize}


\begin{figure}[t!]
	\centering
	\includegraphics[width=0.680\textwidth]{figs/System.pdf}
	\caption{Overview of \FC's architecture~\cite{Nguyen:2019:FRS:3339505.3339636}.}
	\label{fig:Architecture}
\end{figure}


The \FC architecture is depicted in Fig.~\ref{fig:Architecture}. By 
connecting to OSS repositories~\circled{1}, \emph{Code Parser}~\circled{2} 
extracts source code projects to obtain relevant metadata. For each project, 
its source code is also stored to the database for further retrieval. The 
\emph{Data Encoder} component~\circled{3} gets input metadata and represents it in a 
\emph{mathematically computable format}. The similarities among projects, 
declarations are computed by \emph{Similarity Calculator}~\circled{5}. The 
\emph{Recommendation Engine} component~\circled{6} exploits the similarity 
scores and generates recommendations. In particular, \emph{API Generator} 
returns a ranked list of invocations~\circled{7}, whereas \emph{Code Builder} 
queries \emph{Knowledge Base} to get real source code snippets~\circled{8} and  
eventually recommends them to the developer.
%
%
%\subsection{Data Representation}
%
%%We take a concrete example as follows. A software developer is working on the 
%%project \emph{jersey-client-1.18.1}, she has already finished writing $6$ 
%%declarations with $67$ invocations in total. Now the developer is working on 
%%a 
%%new declaration, for this she just added the first API function call, i.e 
%%\code{e.getKey()}. Since Anna is not familiar with the API, she expects 
%%recommendations.
%
%Figure~\ref{fig:MotivatingExample} depicts an example with the Java code 
%snippets of a method declaration named \code{clone()}. For a project, FOCUS 
%works on the basis of declarations and invocations. In the first place, it is 
%necessary to directly extract those artifacts from source code. We chose 
%Rascal 
%M$^3$ \cite{DBLP:journals/corr/IzmaylovaKSV13} since it allows to parse 
%various 
%types of input data. Given a project, the tool is used to extract 
%\emph{relevant} declarations and invocations, i.e. those that come from 
%third-party libraries.   
%
%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=0.680\textwidth]{D6.3_figs/MultivaluedMap.pdf}
%	\caption{Method declaration \textbf{clone()}.}
%	\label{fig:MotivatingExample}
%	%	\vspace{-.4cm}
%\end{figure}
%
%For each declaration or invocation, Rascal M$^3$ returns the full name of data 
%type for all the parameters. Though this seems trivial at first glance, it is 
%useful since it helps distinguish invocations with same name, but containing 
%different types of input parameters. The metadata extracted for the method 
%introduced in Figure~\ref{fig:MotivatingExample} is depicted in 
%Figure~\ref{fig:Declaration}. The declaration is represented as 
%\code{ClientRequestImpl/clone(javax.ws.\-rs.core.MultivaluedMap)} by Rascal 
%M$^3$.%with the parameter \code{javax.w\-s.rs.core.MultivaluedMap}
%
%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=0.680\textwidth]{D6.3_figs/declaration.pdf}
%	\caption{Metadata extracted from \textbf{clone()}.}% 
%	\label{fig:Declaration}
%\end{figure}
%
%From the extracted metadata, we represent the relationships among declarations 
%and invocations using a user-item matrix. In this matrix, each row represents 
%a 
%declaration and each column represents an invocation. A cell is set to $1$ if 
%the declaration in the corresponding row contains the invocation in the 
%column, 
%otherwise it is set to $0$. As an example, Figure~\ref{fig:MD} shows the 
%user-item matrix of project $p_{1}$ with $4$ declarations, i.e. $p_{1} \ni 
%(d_{1}, d_{2}, d_{3}, d_{4})$ and $4$ invocations, i.e. $(i_{1}, i_{2}, i_{3}, 
%i_{4})$.
%
%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=0.30\textwidth]{D6.3_figs/UserItemMatrix.pdf}
%	\caption{Representation of the relationship between declarations and 
%invocations}
%	\label{fig:MD}
%	%	\vspace{-.4cm}
%\end{figure}
%
%%To represent a set of projects,  which aims 
%%\emph{``Active''}
%
%
%To capture the intrinsic relationships among various projects, declarations 
%and invocations, we come up with a 3-D user-item-context matrix. For example, 
%Figure~\ref{fig:3DRepresentation} depicts a set of three OSS projects 
%$P=(p_{a}, p_{1}, p_{2})$ representing by three slices with $4$ declarations 
%and $4$ invocations in total. Project $p_1$ has already been introduced in 
%Figure~\ref{fig:MD} and for the sake of readability, the column and row labels 
%are removed from all the slices in Figure~\ref{fig:3DRepresentation}. There, 
%$p_{a}$ is the \emph{active project} and it has an \emph{active declaration}. 
%\emph{Active} here means the artifact, e.g. project, declaration, being 
%considered/developed. Both $p_{1}$ and $p_{2}$ are complete projects and 
%called 
%\emph{background data} since they are already available and serve as a base 
%for 
%the recommendation process. In practice, it is expected that we can store as 
%much complete projects as possible since the more background data we have, the 
%higher is the possibility we are able to mine relevant invocations.   
%
%
%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=0.80\textwidth]{D6.3_figs/3DMatrix3.pdf}
%	\vspace{-.5cm}
%	\caption{3-D matrix representation of the project-declaration-invocation 
%relationship.}	
%	\label{fig:3DRepresentation}	
%\end{figure}


%===========================================================================================================================================================
%The intuition behind this representation is that, the inclusion of invocations in declarations in a project but in another similar project, we may find a similar inclusion.
%By considering projects as contexts, declarations as users and invocations as items, 
%We consider project as context, declaration as user and invocation as item.
%===========================================================================================================================================================
%A project is considered as a document and method invocation is a term, the similarity between two projects is the similarity between two feature sets.
%we utilize method invocations as features
%Figure~\ref{fig:Similarity} represents. invocation is represented by. In 
% Similarly, t
% among the following pairs. --project, user--declaration, item--invocation. and the following relationships are considered.
%an analogous mechanism for 
% that needs recommendations on which invocations should be further integrated
%By replacing the counterpart, we obtain. 
%===========================================================================================================================================================
%The hypothesis is that if users share the same preference on some items in similar context, then they will likely have the same preference on other common items in other similar context. \hl{Our approach is derived from this to solve the problem of library recommendation}\todo[size=\tiny, color=green!40]{Nr. 16}. Instead of recommending goods or services to customers, we recommend third-party libraries to projects using an analogous mechanism: \emph{``if projects share some libraries in common, then they will probably share other common libraries.''} In a nutshell, we work towards the search for an appropriate answer for the question: \emph{``Which third-party libraries should I further include in my current project?''} Thus, CrossRec aims at supporting software developers who have already included some libraries in the new projects being developed, and expect to get recommendations on which additional libraries should be further incorporated (if any). 
%four projects $(p_{1}, p_{2}, p_{3}, p_{4})$ and four invocations $(i_{1}, i_{2}, i_{3}, i_{4})$ is shown.%by means of the graph.
%There, $p_{a}$ and $p_{1}$ are highly similar since the both point to three nodes namely $(i_{1}, i_{3}, i_{4})$.
%===========================================================================================================================================================

%
%\subsection{Similarity Computation}
%
%By exploiting the collaborative-filtering technique, the presence of 
%additional invocations is deduced from the most similar projects. Given an 
%active declaration in an active project, it is essential to find a set of 
%similar projects, and then most similar declarations in those similar 
%projects. 
%To compute similarities, we exploit the graph representation to model the 
%relationships among projects and invocations introduced in~\cite{8498236}. We 
%employ a similar representation proposed in Section~\ref{sec:CrossSim2}, 
%however using a weighted directed graph. Each node in the graph represents 
%either a project or an invocation, if project $p$ contains invocation $i$, 
%then 
%there is a directed edge from $p$ to $i$. The weight for an edge $p 
%\rightarrow 
%i$ represents the number of invocations $i$ that occur in project $p$. 
%Figure~\ref{fig:Similarity} depicts the graph for the set of projects 
%introduced in Figure~\ref{fig:3DRepresentation}. For instance, $p_a$ has $4$ 
%declarations and all of them have $i_4$ as an invocation. As a result, the 
%edge 
%$p_a \rightarrow i_4$ has a weight of $4$. In the graph, a question mark 
%represents missing information, since for the active declaration in $p_a$, it 
%is not clear if invocations $i_1$ and $i_2$ also belong to it or not.
%
%
%\begin{figure}[h!]
%	\centering
%	%	\vspace{-.4cm}
%	\includegraphics[width=0.60\textwidth]{D6.3_figs/Similarity.pdf}
%	\caption{Graph representation of projects and invocations.}
%	%	\vspace{-.4cm}
%	\label{fig:Similarity}
%	%	\vspace{-.2cm}
%\end{figure}
%
%%To compute the similarities among projects 
%%\cite{DiNoia:2012:LOD:2362499.2362501}, a . 
%
%The similarity between two graph nodes $p$ and $q$ is computed by considering 
%their feature sets \cite{DiNoia:2012:LOD:2362499.2362501}. Given that $p$ has 
%a 
%set of neighbour nodes $(i_{1},i_{2},..,i_{l})$, the features of $p$ are 
%represented by a vector 
%$\overrightarrow{\phi}=(\phi_{1},\phi_{2},..,\phi_{l})$, with $\phi_{k}$ being 
%the weight of node $i_{k}$. It is computed as the \emph{term-frequency inverse 
%document frequency} value as follows: 
%
%%\begin{equation} \label{tfidf} %\nonumber 
%%w_{l}^{d} =tf\cdot idf(l,d,D)= f_{i_k}^{d}\cdot log\frac{n}{\left | \left \{ 
%%d\in D: t_{l} \in d \right \} \right |} 
%%\end{equation}
%
%
%\begin{equation}\label{eqn:TFIDF2}
%\phi_{k} = f_{i_{k}}*log(\frac{ \left | P \right |}{a_{i_{k}}})
%\end{equation}
%
%
%where $f_{i_{k}}$ is the number of occurrence of $i_{k}$ with respect to $p$, 
%it is the weight of the edge $p \rightarrow i_k$; $\left | P \right |$ is the 
%number of projects in the collection; $a_{i_{k}}$ is the number of projects 
%connecting to $i_{k}$. Eventually, the similarity between two projects $p$ and 
%$q$ with their corresponding feature vectors 
%$\overrightarrow{\phi}=\{\phi_{k}\}_{k=1,..,l}$ and 
%$\overrightarrow{\omega}=\{\omega_{j}\}_{j=1,..,m}$ is computed as given 
%below:%\todo[size=\tiny, color=green!40]{Nr. 3}
%%\vspace{-.2cm}
%
%\begin{equation} \label{eqn:VsmSim}
%sim_\alpha(p,q)=\frac{\sum_{t=1}^{n}\phi_{t}\times 
%\omega_{t}}{\sqrt{\sum_{t=1}^{n}(\phi_{t})^{2} }\times 
%\sqrt{\sum_{t=1}^{n}(\omega_{t})^{2}}} 
%\end{equation}
%
%The similarities among method declarations are calculated using the Jaccard 
%similarity index as given below:
%
%\begin{equation} \label{eqn:Jaccard}
%sim_\beta(d,e)=\frac{|\mathbb{F}(d)\bigcap 
%\mathbb{F}(e)|}{|\mathbb{F}(d)\bigcup \mathbb{F}(e)|} 
%\end{equation}
%
%where $\mathbb{F}(d)$ and $\mathbb{F}(e)$ are the sets of invocations of 
%declarations $d$ and $e$, respectively.% contains. 
%
%For instance, in Figure~\ref{fig:3DRepresentation} there is an active project 
%$p_a$ with an active declaration located at the bottom of the matrix, marked 
%with a rectangle. By performing the similarity computation, we obtain 
%$sim_\alpha(p_a,p_1)=0.8$ and $sim_\alpha(p_a,p_2)=0.3$. Furthermore, by using 
%Eq.~\ref{eqn:Jaccard} we find two similar declarations to the active one, and 
%they are also marked with a rectangle in $p_1$ and $p_2$. The similar projects 
%and 
%declarations are used to compute a score for the missing cells. We are going 
%to 
%describe this process in the next section.
%
%%There are two similar projects to $p_a$, i.e. $p_1$ and $p_2$. 
%
%\subsection{API function calls recommendation}
%
%In Figure~\ref{fig:3DRepresentation}, the active project $p_{a}$ already 
%includes 
%three declarations, and the developer is working on the fourth declaration 
%which corresponds to the last two-dimensional matrix. $p_{a}$ consists of only 
%two invocations, represented as the last two columns of the matrix, the cells 
%with the value of $1$. The first two cells are marked with a question mark 
%($?$), indicating that it is not clear whether these two invocations should 
%also be incorporated into $p_{a}$. This simulates a real development scenario 
%where the developer just started working on a new function, she has added two 
%function calls and now expects recommendations on additional invocations. This 
%is the point where FOCUS comes into play. The recommendation engine attempts 
%to 
%predict which invocations the active declaration should include by computing 
%the missing ratings in the corresponding slice (two-dimensional matrix) by 
%means of the following formula \cite{Chen:2005:CCF:2154509.2154540}:% is used 
%%to compute the 
%%weight for each cell
%
%
%
%\begin{equation} \label{eqn:missingRating}
%r_{d,i,p} = \overline{r}_{d} + \frac{\sum_{e \in 
%topsim(d)}(R_{e,i,p}-\overline{r}_{e}) \cdot sim_{\beta}(d,e)}{\sum_{e \in 
%topsim(d)}sim_{\beta}(d,e)}
%\end{equation}
%
%Equation~\ref{eqn:missingRating} is used to compute a real score for the cell 
%representing method invocation $i$ in declaration $d$ of project $p$; 
%$topsim(d)$ is the set of top similar declarations of $d$; $sim_{\beta}(d,e)$ 
%is the similarity between $d$ and declaration $e$, computed using 
%Eq.~\ref{eqn:Jaccard}; $\overline{r}_{d}$ and $\overline{r}_{e}$ are average 
%ratings of $d$ and $e$, respectively. $R_{e,i,p}$ is understood as the 
%combined 
%rating of declaration $d$ for invocation $i$ in all similar projects. It is 
%computed as given below  \cite{Chen:2005:CCF:2154509.2154540}: %using the 
%%following formula: %
%
%\begin{equation} \label{eqn:combinedRating}
%R_{e,i,p}=\frac{\sum_{q \in topsim(p)}r_{e,i,q} \cdot 
%sim_{\alpha}(p,q)}{\sum_{q \in topsim(p)}sim_{\alpha}(p,q)} %\sum_{x \in C}
%\end{equation}
%
%
%where $topsim(p)$ is the set of top similar projects of $p$; 
%$sim_{\alpha}(p,q)$ is the similarity between $p$ and a similar project $q$, 
%computed using Eq.~\ref{eqn:VsmSim}. Equation~\ref{eqn:combinedRating} implies 
%that more weight is given to project with a higher similarity. That means the 
%combined rating for a cell in the active project is more affected by those 
%from 
%the most similar projects. In practice, it is reasonable since given a 
%project, 
%its similar projects seem to contain more relevant API function calls than 
%less 
%similar projects. Using Eq.~\ref{eqn:missingRating} we are able to compute all 
%the missing ratings in the active project and obtain a ranked list of 
%invocations with scores in descending order. The list is then provided to the 
%developer as recommendations.
%
%
%
%%====================================================================================================================================
%%Thus, it is more sensible to mimic the invocation usage in those projects. 
%
%%The intuition behind the 3-D representation is that, given a declaration in a 
%%project, in the ideal case, we can find a project that is exactly the same 
%%as. 
%%In this case, we just need to.
%%We use all the recommended invocations as query, and search against the 
%%database to get the declarations that share.
%% A similarity function that takes into account the sequence as well as the 
%%difference in every position.
%%To recommend concrete source code snippets, it is necessary to .  from the 
%%ranked list of recommendations
%%From the list of items, we reconstruct the correct sequence of a declaration 
%%and eventually retrieve actual code snippets stored in the database. 
%%====================================================================================================================================
%
%
%
%
%
%
%
%\subsection{API usage patterns recommendation}
%
%\paragraph{Using FOCUS} The ranked list of items provided by FOCUS is 
%suggested as the outcome of the recommendation engine. However, it is up to 
%developers to decide how those invocations shall be included. On one side, 
%this 
%scheme gives developers freedom to proceed with the integration process. On 
%the 
%other side, it does not provide enough details to realize a runnable method. 
%In 
%this sense, this type of recommendations might be suitable only for 
%resourceful 
%developers. Thus, to further facilitate the development activities, we also 
%implement a tool for recommending real code snippets.
%
%From the ranked list of recommendations, the \emph{top-N} items are selected 
%and used as query to search the database for relevant declarations. The 
%Jaccard 
%index is used to compute similarity between a set of query items and a 
%declaration represented by metadata consisting set of invocations stored in 
%the 
%Knowledge Base (see Eq.~\ref{eqn:Jaccard}). For each query, we search for 
%declarations that contain as many of the invocations in the query as possible. 
%Eventually, the original source code corresponding to the matched metadata is 
%retrieved from the Knowledge Base and recommended to the developer. %This is 
%%done%The complete code snippet.
%
%%========================================================================================
%%This approach, described in Figure 2, exploits the CLAMS work, in particular 
%%the patterns extracted as output, plus the code cloning features provided by 
%%Simian. 
%%besides the one exploiting FOCUS to recommend code snippets, 
%% which is proposed 
%%and a set of API usage patterns provided by CLAMS. Simian is used to compute 
%%the similarities among the input file and the patterns stored in the 
%%Knowledge 
%%Base. The most similar code snippets are then suggested to the developer.
%%developed by \emph{Katirtzis et. al.} 
%%========================================================================================
%
%
%%============================================Here we introduce the approach 
%%with CLAMS and 
%%SIMIAN===========================================================
%
%
%\begin{figure}[h!]
%	\centering
%	
%\includegraphics[width=0.80\textwidth]{D6.3_figs/APIUsagePatternSimianCLAM.pdf}
%	%	\vspace{-.5cm}
%	\caption{API usage patterns recommendation using a combination of CLAMS and 
%Simian.}	
%	\label{fig:APIUsagePatternSimianCLAM}	
%\end{figure}
%
%
%
%\paragraph{Using CLAMS and Simian} To further enrich the Knowledge Base with 
%various recommendation options, we propose an approach to suggest API usage 
%patterns. The process applied to generate usage patterns is shown in 
%Figure~\ref{fig:APIUsagePatternSimianCLAM}. Open source projects are scraped 
%and 
%used as input for the \code{Code Parser} which then extracts metadata. From 
%this data, CLAMS \cite{10.1007/978-3-319-89363-1_11} is applied to find API 
%usage patterns. As input for the recommendation process, the context where the 
%developer is working on (represented as a file containing source code) is fed 
%to the system. Using 
%Simian\footnote{\href{https://www.harukizaemon.com/simian/}{https://www.harukizaemon.com/simian/}},
%the code is matched against the patterns generated by CLAMS to find the most 
%similar patterns. After this phase, a ranked list of usage patterns is 
%presented to the developer.
%
%
%
%This recommendation tool has been successfully integrated into the Knowledge 
%Base and is available as a REST API.

%========================================================================================================================================================================
%About input files that are necessary to initialise the tool, we have from one side the developer's file with the real snippet of code that he is implementing and may want support for this. On other hand, there are patterns mined by CLAMS, in form of ranked Java files sorted by rational specified in CLAMS paper.
%These file contains patterns, defined as sequence of API method calls that define, instantiate and using class belonging to the APIs contained in the developer'string. The number of these file and also their dimensions in term lines of code depend on the considered libraries. As Simian is a tool based on file comparison, I need to use temporary files of Java to do the comparison; after the process, the files are destroyed. 
%So, at the beginning of the process, we have the patterns files and the devoper's file, represented by a single string. Notice that with this method we keep trace on the context in which the user is developing. Then, all these files is used to extract the recommendations in form of patterns by using Simian integrated in Eclipse platform, following options that I specify in next sections. Basically, at the of this phase, Simian retreives the cloned clone between the developer's file and the CLAMS patterns related to the library that the user is implemented. By using these file, I perfom recommendations by remove the cloned part and suggest to the user the new lines of code that represent the missing pattern for the user. In next sections, I going in deep to describe the entire system and how the integration of Simian and CLAMS works in practise. 
%the intersection of the two sets is maximum. 
%========================================================================================================================================================================
%\subsection{Dataset}
%he dataset is divided into \emph{training data} and \emph{testing data} . 
%Being different from other existing studies which rely on a user study to evaluate the performance of API usage patterns recommendation, we automatize the process by using the ten-fold cross validation technique, 
%========================================================================================================================================================================
%By performing the evaluation with the consideration of the quality metrics previously introduced, we aim at addressing the following research questions: %we want to address in the scope of this paper are the following: %We address three research questions as follows:
%\begin{itemize}
%	\item \textbf{RQ1:} \emph{The performance of FOCUS in comparison to that of CLAMS?} 	%apiAdvisor
%	\item \textbf{RQ2:} \emph{How well can LibRec and CrossRec recommend third-party libraries with regards to accuracy, sales diversity, and novelty?}
%\end{itemize}
%In the next section, the outcomes of the performed evaluation are analyzed and the answers for such research questions are also given.
%. We collect a dataset from the Maven repository
%========================================================================================================================================================================
%
%\smallskip
%
%
%\subsection{Evaluation}
%
%Performing a user study has been accepted as the \textit{de facto}  method to 
%validate an API usage recommendation tool 
%\cite{Moreno:2015:IUT:2818754.2818860,Niu:2017:AUP:3104915.3104977,10.1007/978-3-642-03013-0_15}.
%Nevertheless, such a user study is not only cumbersome but also highly 
%susceptible to errors and individual perception. We introduce a validation 
%approach that automates the evaluation by relying solely on data. We simulate 
%a 
%real developer at different stages of the development process on a dataset 
%curated from OSS repositories beforehand. The following subsections explain 
%the 
%evaluation in more detail.% process.
%
%\subsubsection{Datasets} 
%
%A set of $3.600$ jar files was randomly collected from the Maven 
%repository\footnote{\href{https://mvnrepository.com/}{https://mvnrepository.com/}}
%and named as \code{\textbf{Dataset$\#1$}}. The \code{Data Parser} is used to 
%extract relevant metadata from the projects. However, declarations that 
%contain 
%less than $8$ invocations are discarded. Our assumption is that declarations 
%with a low number of invocations are not helpful and shall not be considered. 
%We checked \code{\textbf{Dataset$\#1$}} manually and noticed that many 
%invocations originate from a same project, i.e. they differ only in their 
%version numbers. For instance, \emph{ant-1.6.5.jar} and \emph{ant-1.9.3.jar} 
%are actually different versions of project \emph{ant}. The 
%collaborative-filtering technique works well given that highly similar 
%projects 
%exist, since it just ``copies'' invocations from similar methods in the very 
%similar projects (see Eq.~\ref{eqn:missingRating}). Since too similar projects 
%may introduce a bias against the recommendation process, we decided to create 
%a 
%second dataset. From \code{\textbf{Dataset$\#1$}}, for projects with same 
%prefix but different version numbers, we randomly selected only one among them 
%and removed all the others. The removal results in a dataset consisting of 
%$1.600$ and we named it \code{\textbf{Dataset$\#2$}}. Evaluation is performed 
%on both datasets to see how well FOCUS recommends API invocations with respect 
%to different input data.  
%
%\subsubsection{Methodology}
%
%By using the datasets, we are able to validate the usefulness of the tool 
%without 
%resorting to a manual analysis of the recommendation outcome. A dataset is 
%split into \emph{training data} and \emph{testing data} and ten-fold cross 
%validation is conducted to validate the performance of FOCUS 
%\cite{Cremonesi:2008:EMC:1468165.1468327}. In particular, the dataset is 
%split in 
%\textit{N} independent sets, \textit{N-1} sets are used for training and 1 for 
%test. The experiment is repeated 10 times, each using a different set for 
%test. 
%The results are averaged over \textit{N}.   This scheme allows us to 
%perform evaluation even on larger datasets.
%
%%====================================================================================================================================
%%as well as a obtaining more precise. 
%%Instead of considering only one active project, we consider by using training 
%%data. In practical use, Training data is the data available for use, whereas 
%%testing data is. Normally, the testing data is divided into two parts, one 
%%part 
%%is used to.
%%FOCUS is able to return match items.
%%\subsection{Discussions}
%%FOCUS is able to find suitable invocations even when only there is a limited 
%%number of declarations available.
%%We conduct a series of experiments corresponding to different development 
%%phases using ten-fold cross validation as it is considered as one of the best 
%%methods for model selection \cite{Kohavi:1995:SCB:1643031.1643047}. The 
%%dataset 
%%is divided into ten parts and the validation is performed in 10 rounds.
%%====================================================================================================================================
%
%%====================================================================================================================================
%% whereas later on, the number of declarations
%%Only \emph{top-N} invocations are used for evaluation.
%%Given a testing project, there are two parameters to be considered: the first 
%%is the number of method declarations it contains denoted as $\#dec$, and the 
%%second parameter is the number of invocations the testing declaration 
%%currently 
%%contains $\#inv$.
%
%%All the written declarations together with the invocations in the active 
%%declaration are considered as context data for the recommendation. At an 
%%early 
%%stage, $\#md$ and $\#mi$ are small and. Intuitively, the more context data 
%%there is, the easier it is to find suitable method invocations.
%%We consider the following test configurations: Each project consists of 
%%method declarations, and each declaration has a number of invocations. The 
%%training projects are used to. For a testing project, i.e. the one that needs 
%%recommendation, a method declaration is randomly selected as testing and we 
%%call this the active method. For the active method declaration, only one 
%%method 
%%invocation is fed to the system. Different settings: using all method 
%%declarations, using only one method invocation and using some method 
%%invocations.
%%to see if the system is able to
%%We perform experiments using different configurations. 
%%\#inv/2
%%====================================================================================================================================
%
%
%\begin{table*}[h!]
%	\scriptsize
%	\centering	
%	\begin{tabular}{|p{0.50cm}|p{6.80cm}||p{0.55cm}|p{6.9cm}|}  
%		\hline				
%		%& 
%%\multicolumn{1}{|c||}{\textbf{\href{https://github.com/guoguibing/librec}{guoguibing/librec}}}
%% & \multicolumn{2}{c|}{\textbf{Recommendations}}  \\ 
%%\hline								
%		& \emph{\textbf{Invocations}} & \emph{\textbf{Rank}} &  
%\emph{\textbf{FOCUS}}  \\  \hline		
%		{\multirow{9}{*}{\rotatebox[origin=c]{90}{Ground-truth}}} & 
%org.json4s.package\$.JObject() 	& 1 &  
%\textbf{scala.collection.immutable.List.map(scala.Function1,scala\-.collection.generic.CanBuildFrom)}
%   \\ \cline{2-4}   			
%		& 
%org.json4s.native.JsonParser\$\$anonfun\$1\$\$anon\-fun\$org\$json4s\$native\$JsonParser\$\$anonfun\$\$reverse\-\$1\$2/2(org.json4s.native.JsonParser\$\$anonfun\$1)
%	 & 2 &  \textbf{scala.collection.immutable.List\$.canBuildFrom()}   \\ 
%\cline{2-4}		
%		& scala.collection.immutable.List.reverse()	 & 3 &  
%\textbf{org.json4s.JsonAST\$JArray.arr()}   \\ \cline{2-4}	
%		& 
%scala.collection.immutable.List.map(scala.Function1,sca\-la.collection.generic.CanBuildFrom)
%   & 4 & scala.Option.isEmpty()   \\ \cline{2-4}				
%		& 
%org.json4s.JsonAST\$JObject\$.apply(scala.collection.immu\-table.List)  & 5 &  
%scala.collection.immutable.Map\$.apply(scala.collection.Seq)    \\ 
%\cline{2-4}			
%		& org.json4s.JsonAST\$JArray\$.apply(scala.collection.immu\-table.List) 
%& 6 &	
%org.json4s.package\$MappingException.MappingException(ja\-va.lang.String) \\ 
%\cline{2-4}
%		
%		& org.json4s.JsonAST\$JArray.arr()  & 7 &  
%scala.collection.mutable.StringBuilder.StringBuilder()   \\ 
%\cline{2-4}					
%		& scala.collection.immutable.List\$.canBuildFrom()  & 8 &  
%\textbf{org.json4s.package\$.JObject()}  \\ \cline{2-4}		
%		& org.json4s.package\$.JArray()  & 9 & 
%java.lang.Object.equals(java.lang.Object) \\ \hline					
%		{\multirow{1}{*}{\rotatebox[origin=c]{90}{Testing}}}  & 
%		org.json4s.JsonAST\$JObject.obj()  & 10 & 
%		
%\textbf{org.json4s.JsonAST\$JObject\$.apply(scala.collection.imm\-utable.List)}
%		\\ \hline		
%	\end{tabular}
%	\caption[Summary]{Example of recommendation results.}
%	%	\vspace{-.6cm}
%	\label{tab:APIFunctionCallsEx}
%\end{table*}
%
%Table~\ref{tab:APIFunctionCallsEx} gives an example of recommendation results 
%provided by FOCUS. On the left side of the table, there are all invocations of 
%an active declaration. We keep only one invocation as testing data and take 
%out 
%the others and use as ground-truth data. On the left side of table, there are 
%\emph{top-10} items recommended by FOCUS. Among $10$ retrieved items, $5$ of 
%them are found in the ground-truth data. The example shows that FOCUS is able 
%to retrieve relevant invocations, given that only one invocation is available 
%as input data.
%
%We simulate different stages of a real development process to study if the 
%system is applicable, considering a programmer who is developing a software 
%project $p$. At the point of consideration, the developer already finished a 
%number of method declarations $\delta$, and she is now working on the active 
%declaration $d_a$. For this function, the developer has just finished writing 
%a 
%specific number of invocations, let's say $\pi$, and she has to complete 
%$d_a$. 
%The two parameters $\delta$, $\pi$ are used to stimulate different stages of 
%the development process. In practice, $\delta$ is low at an early stage and 
%increases over the course of time. From a recommender system point of view, we 
%expect to provide the developer with suitable suggestions that match the 
%context well in various phases.
%
%To thoroughly evaluate the performance of our proposed approach, we utilize 
%ten-fold cross validation \cite{Kohavi:1995:SCB:1643031.1643047}. A dataset 
%is split into $10$ equal parts, i.e. \emph{folds}, and an evaluation is 
%conducted in $10$ rounds. In each round of validation, nine folds are used for 
%training and the remaining fold is for testing. Given a testing project, we 
%call the number of method declarations as $\#dec$ and we conduct a preliminary 
%evaluation by considering the following configurations:%, and the second 
%%parameter is the number of invocations $\#inv$
%
%
%\paragraph{\textbf{Configuration Conf\#1:}} $\delta=\#dec/2$-$1$, $\pi=1$. One 
%declaration is used as testing data, only half of the remaining declarations 
%are used as training data and the other half are removed. For the testing 
%declaration, only one invocation is provided as input for recommendation, and 
%the rest is used as ground-truth data. This configuration mimics a scenario 
%when the developer is at an early stage of the development process and 
%therefore, only limited context data is available for feeding the 
%recommendation engine.
%
%\paragraph{\textbf{Configuration Conf\#2:}} $\delta=\#dec$-$1$, $\pi=1$. One 
%method declaration is selected as testing data, all the remaining declarations 
%are used as training data. Similar to \code{\textbf{Conf\#1}}, by the testing 
%declaration only one invocation is kept and all the others are taken out to 
%use 
%as ground-truth data. This represents the stage when the developer almost 
%finishes implementing the project.
%
%It is expected that the proposed system can recommend items that eventually 
%match with those stored as ground-truth data.
%
%\begin{figure*}[h!]
%	\label{fig:SuccessRateFOCUS}
%	%	\vspace{-.4cm}
%	\begin{tabular}{c c}	
%		%		\vspace{-.5cm}
%		\centering    
%		\subfigure[Success rate for 
%Dataset\#1]{\label{fig:SuccessRate3600}\includegraphics[width=0.45\textwidth]{D6.3_figs/SuccessRateD3600.pdf}}
%		& 	
%		\subfigure[Success rate for 
%Dataset\#2]{\label{fig:SuccessRate1600}\includegraphics[width=0.45\textwidth]{D6.3_figs/SuccessRateD1600.pdf}}\\
%	\end{tabular}	
%	\caption{Success rate.}
%	%	\vspace{-.4cm}
%\end{figure*}
%
%
%\subsection{Result Analysis}
%
%Figure~\ref{fig:SuccessRate3600} and Figure~\ref{fig:SuccessRate1600} depict 
%the success rate obtained for different cut-off values, i.e. $N=\{1, 5, 10, 
%15, 
%20\}$ for both configurations \code{\textbf{Conf\#1}} and 
%\code{\textbf{Conf\#2}}. We investigate the outcome by each dataset, i.e. 
%\code{\textbf{Dataset$\#1$}} and \code{\textbf{Dataset$\#2$}} separately. 
%Interestingly, there are no big differences in success rate between two 
%configurations for all values of $N$. This demonstrates that FOCUS is able to 
%generate relevant recommendations also when only limited context data is 
%available. By comparing the two figures we see that FOCUS produces better 
%matches given that more similar projects are available, as in 
%\code{\textbf{Dataset$\#1$}} there exist projects with different version 
%numbers.
%
%For a small $N$, i.e. $N=1$, that means when the developer expects a very 
%brief list of recommendations, the system is still able to provide matches. 
%For 
%example, with \code{\textbf{Dataset$\#1$}}, the success rates of 
%\code{\textbf{Conf\#1}} and \code{\textbf{Conf\#2}} are $72.30\%$ and 
%$72.80\%$, respectively. Meanwhile, the outcome by 
%\code{\textbf{Dataset$\#2$}} 
%is much lower for both configurations with $N=1$, the success rates of 
%\code{\textbf{Conf\#1}} and \code{\textbf{Conf\#2}} are $49.40\%$ and 
%$50.10\%$, respectively. This suggests that the performance of FOCUS improves 
%considerably, given that more similar projects are available.
%
%\begin{figure*}[h!]
%	%	\vspace{-.4cm}
%	\begin{tabular}{c c}	
%		%		\vspace{-.5cm}
%		\subfigure[Precision and recall for 
%Dataset\#1]{\label{fig:PrecisionRecall3600}\includegraphics[width=0.45\textwidth]{D6.3_figs/PrecisionRecall_D3600_Fold10.pdf}}
%		& 	
%		\subfigure[Precision and recall for 
%Dataset\#2]{\label{fig:PrecisionRecall1600}\includegraphics[width=0.45\textwidth]{D6.3_figs/PrecisionRecall_D1600_Fold4.pdf}}
%		\\
%		%		\vspace{-.3cm}
%	\end{tabular}
%	\label{fig:Accuracy}
%	\caption{Accuracy.}
%	%	\vspace{-.4cm}
%\end{figure*}
%
%
%Next, we investigate the accuracy of both configurations by varying the 
%cut-off value $N$ from $1$ to $30$ to get $Precision@N$ and $Recall@N$ and 
%sketch the Precision-Recall curves as shown in 
%Figure~\ref{fig:PrecisionRecall3600} and Figure~\ref{fig:PrecisionRecall1600}. 
%Considering \code{\textbf{Dataset\#1}}, we witness the same trend as by 
%success 
%rate, since there are no big distinctions between accuracies for the 
%configurations with all cut-off values $N$. Only a small difference in the 
%accuracy of \code{\textbf{Conf\#1}} and \code{\textbf{Conf\#2}} can be seen in 
%\code{\textbf{Dataset\#1}}. With this dataset, \code{\textbf{Conf\#2}} has a 
%better accuracy as the corresponding curve is closer to the top right corner. 
%It is understandable since by \code{\textbf{Conf\#2}}, there is more 
%background 
%data available for recommendation.  
%
%The experimental results show that FOCUS recommends API function calls with 
%high success rates. 
%Nevertheless, the performance of FOCUS needs to be further studied through 
%additional experiments 
%considering various configurations. This is considered as a future work and we 
%will be back to fully 
%investigate the use cases in Deliverable D6.5. %This is an ongoing work and 
%
%
%
%
%%To match this set of invocations against the database, a similarity function 
%%needs to be defined. The function has to take into account the presence as 
%%well 
%%as the sequence of API invocations. To this end, we decided to choose the 
%%Levenshtein distance \cite{Levenshtein_SPD66} since it meets the defined 
%%requirements. Considering a declaration, every invocation is encoded using a 
%%unique character. Also the list of top-N recommended items is encoded using a 
%%string. In this way, we can measure the similarity between a \emph{top-N} 
%%list 
%%and a declaration by computing the Levenshtein distance between their 
%%corresponding strings, taking into account the presence and sequence of the 
%%invocations. The scores are used to produce a ranked list of source code 
%%examples. $N$ can be changed according to number of invocations a declaration 
%%in the database contains. Finally, we extract concrete code examples from 
%%source code projects.%\cite{Moreno:2015:IUT:2818754.2818860}. 
%
%
%\smallskip
%
%%==================================================================================================================================
%%First search for. In this paper, we propose CodeAdvisor, a framework for 
%%recommending suitable API function calls to a given project being developed. 
%%Given a method declaration, Method invocations 
%%==================================================================================================================================
%%\subsection{API function calls recommendation}
%%
%%The representation in Figure~\ref{fig:3DRepresentation} allows to model the 
%%relationships among projects, declarations and invocations. In 
%%Figure~\ref{fig:3DRepresentation}, the active project $p_{a}$ already 
%%includes 
%%three declarations, and now its developer is working on the 4th declaration. 
%%With this function, there are only two invocations, i.e. the cells filled 
%%with 
%%$1$. It is necessary to compute the missing ratings, or to see if the 
%%inclusion 
%%of an invocation. Collaborative here means to deduce the missing values by 
%%looking to the similar projects, at the similar positions to see.
%%
%%To mine API usage patterns from similar projects. Project similarity, method 
%%similarity. To mimic an actual situation when a developer is working on a 
%%method declaration and he already has one or some method invocations, the 
%%engine is expected to provide her with suggestions which method invocations 
%%should be further incorporated. The active project is represented as one 
%%slice, 
%%and the. The following formula is used to compute the weight 
%%\cite{Chen:2005:CCF:2154509.2154540}.
%%\begin{equation} \label{eqn:combinedRating}
%%R_{u,i,c}=\frac{\sum_{x \in C}\sum_{t}^{z}r_{u,i,x} \cdot 
%%sim(c,x)}{\sum_{x}^{y}sim(c,x)}
%%\end{equation}
%
%%$R_{u,i,c}$ is the rating of user $u$ for item $i$ in context $c$. This is 
%%
%%
%%Eq.~\ref{eqn:combinedRating} implies that weight is given to project with 
%%higher similarity. In practice, it is understandable since similar projects 
%%seem to contain similar function calls.
%%
%%The missing rating is computed using the following formula:%as follows:
%%
%%\begin{equation} \label{eqn:missingRating}
%%r_{a,i,c} = \overline{r}_{a} + \frac{\sum_{i}^{n}(R_{u,i,c}-\overline{r}_{u}) 
%%\cdot sim_{J}(a,u)}{\sum_{x}^{y}sim_{J}(a,u)}
%%\end{equation}
%%
%%
%%%Eq.~\eqref{eqn:missingRating} is used to computed a score for the cell 
%%%representing method invocation $i$, declaration $a$ of project $c$.  
%%%$sim_{J}(a,u)$ is the similarity between the active user $a$ and a user $u$
%%
%%
%%
%%\subsection{API usage patterns recommendation}
%%
%%To reconstruct the correct sequence of a function call, we use the top-N 
%%recommended invocations as query to search for relevant. We use all the 
%%recommended invocations as query, and search against the database to get the 
%%method declaration that shares. The scores are used to produce a ranked list 
%%of 
%%source code examples. A similarity function that takes into account the 
%%sequence as well as the difference in every position. We decided to choose 
%%the 
%%Levenshtein distance. Considering a declaration, every invocation is encoded 
%%using a character. Also a list of top-N recommended invocations is encoded 
%%using a string. In this way, we can measure the similarity between a ranked 
%%list and a declaration by computing the Levenshtein distance between their 
%%corresponding strings.
%%
%%the intersection of the two sets is maximum. 
%



==> src/Lessons.tex <==
Developing the \CM \rs has been a long journey, which allows us to 
garner many useful experiences. These experiences are valuable resource, which we can rely on in the future whenever we are supposed to run similar projects. In the following paragraphs, we discuss in detail the main lessons learned through the development of the project. %are singularly discussed.

% Such experiences are useful,

%\nb{Davide}{Organize the discussion of the lessons learned with 
%respect to the three phases, i.e., requirement elicitation, 
%development, and evaluation}

%
%https://dl-acm-org.univaq.clas.cineca.it/doi/pdf/10.1145/2959100.2959194
%
%Users might not trust what you are recommending. You need to explain
%
%
%Requirement elicitation:
%- Important to have concrete examples to be discussed with the final 
%users. Artificial input and outputs can help in this direction.
%
%Development
%- Start with existing approaches. Do not reinvent the wheel.
%- Lavoro certosino, di fino
%
%Evaluation
%
%- Identify and select the baselines with available data sets and 
%tools. 
%
%- It is possible to overcome the problems related to user studies by 
%applying cross-validation techniques
%
%- Precision and recall are the minimal metrics that need to be 
%employed
%
%- Even when the baseline is not available, do not disperate, 
%cross-validation to the rescue
%








==> src/SOrec.tex <==

%API documentation recommendation

%Third-party libraries are interface to runnable and reusable code snippets, they can be embedded in source code projects independently from environment code \cite{Robillard:2013:AAP:2498733.2498776}. 
%to see how API instances are utilized in practice. 
%from these external sources, there are only documentations providing generic syntax or simple usage of the API, which may be less relevant to the current development context. In this sense, concrete examples of source code snippets that drop a hint about how specific API function calls are deployed in actual usage, are of great use \cite{Moreno:2015:IUT:2818754.2818860}.\part{title}
%This means that the lower bound of our dataset will be about 1,422,519 snippets of code and possibly much more if we consider all the answers and comments. 
%The date when the post was created 
%it is also possible to decide which fields save from the dump and which discard.
%Since now this is the parsing flow: (could be changed if needed)
%1 - From the dump xml file we analyse all the posts.
%1.1 - We save the posts where the Code field is NOT EMPTY and where the acceptedAnswerId is 2,
%in such a way we collect all the answers with a code.


%Once a developer has embedded a third-party library in the current project, she also looks for corresponding API documentations that describe the constituent functions, in order to understand how to incorporate them into current code. Consulting external sources such as StackOverflow \cite{Ponzanelli:2014:MST:2597073.2597077} provides the developer with a broader insight of API usage, and in some cases, with sound code examples. Nevertheless, as the information space is huge, it is necessary to have tools that help narrow down the search scope as well as find the most relevant documentations. In this chapter, we introduce an approach to filter out low quality and irrelevant StackOverflow posts, aiming to recommend useful items. Given some API function calls the developer has already included, our tool allows to retrieve messages from StackOverflow posts that can give more insight into the application of the APIs.
%In this chapter, we are going to address the use case \textbf{GetAPIUsageDiscussions} depicted in Figure~\ref{fig:Recommendations}.

% that are useful for understanding how to properly use it \cite{Ponzanelli:2014:MST:2597073.2597077}
%. Only those that contain good code are suitable for the recommendation.


During the development of complex software systems, programmers look 
for external resources to understand better how to use specific APIs 
and to get advice related to their current tasks. 
StackOverflow provides developers with a broader insight of API 
usage and with useful code examples. However, finding 
StackOverflow posts that are relevant to the current context is a 
strenuous task~\cite{5287006}. In this section, we introduce \SR, an approach that 
allows developers to retrieve messages from StackOverflow being relevant to the API function calls that they have already defined, 
as well as to the external libraries included in the project being 
developed.

The approach has been validated by means of a user study 
involving 11 developers who evaluated 500 posts with respect to 
50 contexts. Experimental results indicate the suitability of \SR to 
recommend relevant StackOverflow posts and concurrently show that the tool 
outperforms a well-established baseline.
%We implement a system for recommending SO posts, \ie~SOrec (see Section~\ref{sec:SOrec}). 








\subsection{Overview}


Developing complex software systems requires mastering several 
languages and technologies
\cite{robillard_recommendation_2014}. 
Consequently, software developers need to continuously devote effort to 
understand how to use new third-party libraries even by consulting 
existing source code or heterogeneous sources of information. 
The time spent on discovering useful resources can have a 
dramatic impact on productivity 
\cite{Duala-Ekoko:2012:AAQ:2337223.2337255}. 

%
%The development of a complex software systems necessitates 
%considerable efforts from developers, and often they 
%tackle 
%various issues related to integration tasks. For instance, 
%developers frequently have the need to integrate new API 
%methods coming from third-party libraries which may not be 
%familiar to them. To understand how to invoke these 
%methods 
%properly, they have to consult external sources that 
%provide additional documentations. 
%
%Among others, StackOverflow (SO)~\cite{stackoverflow} is a 
%good source of support and it is frequently visited by 
%developers~\cite{ABDALKAREEM2017148,Linares-Vasquez:2014:ACT:2597008.2597155}.

A recent work shows that StackOverflow 
(SO)~\cite{stackoverflow} is the most popular 
question-and-answer website \cite{Baltes2018}, which is a 
good source of support for developers who 
seek for probable solutions from the Web 
~\cite{ABDALKAREEM2017148,Linares-Vasquez:2014:ACT:2597008.2597155}.
SO discussion posts provide developers with a broader 
insight of API usage, and in some cases, with sound code 
examples. Nevertheless, as the information space is huge, 
it is necessary to have tools that help narrow down the 
search scope as well as find the most relevant 
documentations \cite{robillard_recommendation_2014}. 
However, how to construct a query that best describes the 
developer's context and how to properly prepare SO data to 
be queried are still challenging tasks 
\cite{DBLP:journals/ese/PonzanelliBPOL16}. In particular,  
there is a need to enhance the quality of retrieved posts 
as well as to refine the input context to generate decent 
queries, which then facilitate the search process. 


%\PN{It is necessary to give a more detailed summary for StackOverflow here.}

%===================From this paper: https://soarsmu.github.io/papers/sac13.pdf===================
%\footnote{\url{https://stackoverflow.com/}}
%Software development and maintenance are complex activities
%that often involve many concepts and reference documents.
%Many aspects of the software, such as the interface
%defined, APIs used, bugs fixed, and even architectural designs,
%may be changed over time. In order to work with
%so many aspects and details involved in a software project,
%developers often need helps from one another. A widely
%used way is for developers to ask questions and/or answer
%them in various online forums. StackOverflow is one of the
%most popular question and answer sites [1] for developers.
%Millions of questions are posted there, and many of these
%questions are answered by various developers [16].

%======================================================================================================================================================================
%Thus, it is necessary to find posts that are highly related to the current context.
%developer's context. 
%, which make the matching process become difficult
% and cannot be queried
%In this paper, we propose an approach to.
%. Still there are more challenges. 
%\emph{Cordeiro~\etal} present an approach~\cite{6233418}. 
%We propose a novel approach in this field that exploits 
% to provide the final recommendations.  
% to cope with the above mentioned issues
%limited to the cases when
% is complete and of high quality
% Thus, they cannot deal with posts that contain incomplete, or missing information. 

%\begin{itemize}
%	\item The extracted code snippets are normally incomplete and contain noise.
%	\item The relevance of each code component.
%	\item The execution time is.
%\end{itemize}

% the most notable approach
%applicable only to 


%====================================What has been done so far=========================================================================================================
%======================================================================================================================================================================
%So far, a number of approaches have been proposed to 
%tackle 
%the issue of retrieving posts from SO that are relevant 
%with respect to the current developer context. Among 
%others 
%Prompter~\cite{DBLP:journals/ese/PonzanelliBPOL16} has 
%been 
%implemented to recommend SO posts. However, the tool 
%neglects some important factors, for example code 
%similarity. As we see later on in this paper, the main 
%limitation is the accuracy, sometimes \FC is unable to 
%retrieve results at all or it is not so accurate,~\ie~it 
%suggests the wrong library for some certain contexts. 
%Though the existing tools can provide SO posts, they are 
%limited to complete and high quality background data.
%%=====================================What needs to be done more/What is still missing================================================================================
%======================================================================================================================================================================
%Furthermore, a large number of SO posts normally contain 
%noise and incomplete code snippets. From a human point of 
%view, the contained snippets can still be useful at some 
%extent when they are presented to developers. However, for 
%machines, such posts are considered to be incomplete, and 
%thus hindering the search activities. Specifically, there 
%are the following issues: \emph{(i)} The extracted code 
%snippets are normally incomplete and contain noise; 
%\emph{(ii)} The relevance of each code component; and 
%\emph{(iii)} The execution time is.

%======================================What we are going to solve the problems (Research objectives)===================================================================
%======================================================================================================================================================================

%query 
%In particular, we introduce entropy which is typically used in the information retrieval (IR) context.
%, and also by using a manual evaluation with different query configurations to evaluate the accuracy and the quality of recommended posts
%From the results, we claimed that our approach overcomes \FC in term of quality of the snippets of code as well as the time computation.
%of the query and the quality of obtained results
%the matching process becomes difficult
%. We believe that there is still room for improvement
%eventually 


%In this work 
We propose \SR, a comprehensive approach imposing 
various measures on both the data collection and query 
phases. To improve efficiency, we exploit Apache Lucene 
\cite{lucene}, an information retrieval library to index 
the textual content and code coming from StackOverflow. 
Posts are retrieved and augmented with additional data to 
make them more exposed to queries. On the other side, we boost 
the context code with different factors to construct a 
query that contains information needed for 
matching against the stored indexes. In a nutshell, we make use of \emph{multi facets} of the data available at hand to optimize the search process, with the ultimate aim of recommending highly relevant SO posts. %populate a database and build code queries.
The approach's performance has been assessed by considering various 
experimental settings. We also compare our tool 
against a well-established baseline, 
\ie~\FC~\cite{DBLP:conf/icse/KimKBC0KT18}. Through a series 
of user studies, we demonstrate that our proposed approach 
considerably improves the recommendation performance, and 
thus outperforming the considered baseline. In this sense, we have the following contributions:

%{\bf to be refined}
%\begin{enumerate}
%	\item An approach to augment code queries with additional information that 
%helps populate a complete and informative database.
%	\item Implementation of \SR, a recommender system for providing SO posts.
%	\item A comprehensive evaluation on a dataset collected from an SO dump by 
%means of well-defined user studies.
%\end{enumerate}

\begin{itemize}
	\item Identification of augmentation measures to automatically refine the 
	considered input SO dump by considering various pieces of information;
	\item Exploiting a well-founded IR tool to index the augmented data;
	%, so as to speed up the query answering process.	
	\item Characterizing the context code by automatically boosting the 
	constituent terms to improve their exposure to the indexed data and 
	eventually build a proper query in a transparent manner for the developer;
	\item Two empirical evaluations of the proposed approach to 
	evaluate the performance of \SR and to compare it with \FC.% 
	%so 
	%that. %enhancement (if present);
	%	\item The indexing method;
	%	\item The supported language; 
	%	\item Addition of libraries in the title and body. 
	%	\item Improve the parsing of the code.
	%	\item The introduction of entropy.
	%	\item Lucene with BM25.	
	%	\item Construct query by using original code snippet.
	%	\item Add import information.
	%	\item Using BM25 to encode the input feature.
\end{itemize}


%======================================The paper's structure=================================================================
%other approaches that face the problem of code snippets recommendations and their limitations
% \Cref{sec:ProposedApproach} shows the overall structure of our approach and how we have implemented and integrated the entropy within Lucene.

This chapter is structured into the following sections.~\Cref{sec:SOrecBackground} provides background and describes the motivations for our work. In~\Cref{sec:SOrec}, we introduce \SR, our proposed approach to recommend StackOverflow posts. The evaluation is presented in \Cref{sec:SOrecEvaluation}. \Cref{sec:SOrecResults} analyzes the experimental results. Finally, \Cref{sec:SOrecThreats} discusses the threats to validity.
%\Cref{sec:Threats} discusses the threats to validity. 
%In~\Cref{sec:RelatedWork} we present related work and conclude the paper in~\Cref{sec:Conclusions}.
% the possible improvement and %future challenges in this field.


\subsection{Background and Motivations} \label{sec:SOrecBackground}



Over the last decade several approaches have been 
conceived to leverage the use of crowdsourcing in 
software engineering \cite{MAO201757}. Those 
exploiting StackOverlow as main source of 
information (\eg 
\cite{deSouza2014,DBLP:conf/icse/KimKBC0KT18,6606701,DBLP:journals/ese/PonzanelliBPOL16,6233407})
can be 
distinguished in two main categories:

\begin{itemize}
	
	\item[\textit{C1.}] approaches that pay attention only to the automated creation of queries to be executed by search engines, and to the visualization of the retrieved posts according to some ranking model (\eg \cite{deSouza2014,6606701,DBLP:journals/ese/PonzanelliBPOL16});
	
	\item[\textit{C2.}] approaches that focus both on query creation and on advanced indexing mechanisms specifically conceived for storing and retrieving SO posts (\eg~\cite{DBLP:conf/icse/KimKBC0KT18,6233407}).
	
\end{itemize}


Prompter~\cite{DBLP:journals/ese/PonzanelliBPOL16}  
is among the most recent approaches falling in the 
first category above. It is an automatic tool, 
which is used to recommend SO posts given an input 
context built from source code. Prompter performs 
various processing steps to produce a query. First, 
it splits identifiers and removes stop words. Then 
it ranks the terms according to their frequency by 
considering also the entropy of the term in the 
entire SO dump. Once the query is built, the tool 
exploits a web service to perform the query 
via the Google and Bing search engines. Finally, a 
ranking model is employed to sort the results 
according to different metrics such as API 
similarity, tags analysis, and SO answers and 
questions. 

%Though being capable of providing relevant posts, 
%the main limitation of this approach is that it 
%heavily relies on online queries, searching for 
%possible recommendations from the Web. In this 
%sense, some delays may happen during the 
%recommendation phase. Furthermore, the tool cannot 
%work well with incomplete or noisy data. 

%\FC is a code search engine that exploits 
%StackOverflow to extend original queries. We study 
%the two approaches to 
%understand their strength and weaknesses as 
%follows.


\FC~\cite{DBLP:conf/icse/KimKBC0KT18} is a recent 
code-to-code search engine that relies on Apache 
Lucene %\footnote{\url{https://lucene.apache.org/}} 
and provides developers with relevant  
GitHub code 
snippets. %~\cite{DBLP:conf/icse/KimKBC0KT18}.
Two 
main phases are conducted to produce 
recommendations as follows. The first one is 
performed on the context code to get related SO 
posts from a local indexed dump. To this end, the system 
parses the context code and builds an initial query 
$q_c$ to look for posts from StackOverflow. From 
the set of retrieved posts, it parses natural 
language descriptive terms from questions to match 
against the question index of Q\&A that has been 
built ex-ante in order to get more posts that 
contain relevant source code. Afterwards, a new 
query $q_c'$ is formed from the newly obtained 
source code. The second phase is done on $q_c'$ to 
search from GitHub for more snippets, which are 
finally introduced to developers. 
%
By focusing on the first phase, \ie 
searching for SO posts by exploiting the input 
context code, \FC can be considered in category 
\textit{C2} above. This module works like a bridge 
between the initial query $q_c$ and the final 
results. In this sense, it has an important role to 
play since its performance considerably affects the 
final recommendation outcomes. 

\smallskip
The experimental 
results~\cite{DBLP:conf/icse/KimKBC0KT18} 
demonstrate that \FC obtains a superior performance 
with regards to several baselines. %, \eg Searchcode, Krugle, or Sourcerer. 
%Furthermore, the system is able to retrieve different Type-3 and Type-4 
%clones, 
%which is highly useful. 
In this section we pay our attention only to the \FC's module for 
searching SO posts. By a 
careful observation on the system, we found out 
that it suffers a setback with respect to 
incomplete data as well as brief input query. As we 
can see later on in this chapter, for many queries the system is 
unable to retrieve any SO posts, or for some 
contexts it suggests irrelevant ones, \ie false positives. To this end, we believe that there is a need to overcome the limitations, so as to enhance the overall performance of \FC.

%is not so accurate, \ie 
%from a low performance 
%Thanks to the indexing mechanism provided by Lucene, \FC can provide. Nevertheless, 
%Though the system has been evaluated on. 
%It cannot work well with incomplete. 
%As we can see later in the paper sometimes
%The main limitation is the accuracy, a
%This aims at expanding the original query to yield 
%since it plays an important role since 
%\ie the SO module of \FC 
%By the first phase, uses Lucene to build and perform a query on an SO dump. 
%The aim is to find similar posts on SO considering the semantic and not only the syntactic structure of the snippet of code. 
%To this end, Lucene is exploited to set indexes that represent the relationship between the code and the semantic. In particular, \FC uses the snippet index to associate the answer document IDs with the code in the SO posts, by creating pairs in form of token\_type: actual\_token with Lucene.
%%To generate all possible terms from the code, the authors parse the AST of the code, by wrapping the incomplete code in a dummy class if needed.
%The second index, called question index, maps the information between the question and the source code in the SO posts.
%\FC uses this index to perform semantic analysis and try to find alternate queries that should cover more cases. Finally, \FC uses the code index to search the similarity between the user's code and the code in the SO posts. The tool builds the AST of the code (building dummy classes if needed), similarly with respect to the first index. Once the authors define these indexes, \FC retrieves the results and, by using Lucene functions, it ranks the results. In particular, the tool exploits the Lucene function for textual similarities like Boolean Model and Vector Space model for scoring, plus TF-IDF for rank the result and to compute the Cosine similarity between the developer's code and indexed snippets. As the final recommendations, it produces code snippet coming from GitHub by using a local dump already crawled.
% depicts a relevant post from StackOverflow
% However, \FC fails to retrieve posts for this example. By running.
%Unfortunately, \FC fails to return any results.

%\footnote{\url{https://tinyurl.com/y6bsmo4z}}
As an example, we consider the explanatory code snippet shown in 
Listing~\ref{lst:OriginalCode}. The code declares a 
\code{CamelContext} variable, and invokes functions 
\code{addRoutes()} and \code{configure()}. The 
input code is pretty simple, and the developer 
would benefit from being suggested with SO posts discussing 
aspects related to the input source code.
%
%\begin{figure}[t!]
%	\centering	
%	\includegraphics[width=0.45\textwidth]{figs/MotivatingExample.png}
%	\vspace{-.4cm}
%	\caption{Explanatory input context code.}
%	\vspace{-.4cm}
%	\label{fig:OriginalCode}
%\end{figure}

	%
	\begin{lstlisting}[caption={Explanatory input context code.}, label=lst:OriginalCode,captionpos=b,style=JavaStyle,numbers=left,xleftmargin=2em,frame=single,framexleftmargin=1.5em]
	package camelinaction;
	
	import org.apache.camel.CamelContext;
	import org.apache.camel.builder.RouteBuilder;
	import org.apache.camel.impl.DefaultCamelContext;
	
	
	public class FilePrinter {
	
	   public static void main(String args[]) throws Exception {
   	      // create CamelContext
 	      CamelContext context = new DefaultCamelContext();
	
	      // add our route to the CamelContext
	      context.addRoutes(new RouteBuilder() {
	      public void configure() {
	
	      }
	    });
	  }
	}
	\end{lstlisting}
% 

In other words, it is expected that a search engine can recommend 
discussions that are relevant to the developer context, for 
instance the 
post\footnote{\url{https://tinyurl.com/yydp8lwd}} 
shown in Figure~\ref{fig:RecommendedPost}. 
\begin{figure}[h!]
	\centering	
	%	\vspace{-.1cm}
	\includegraphics[width=0.68\textwidth]{figs/RecommendedPost.png}
	%	\vspace{-.4cm}
	\caption{A StackOverflow post that is relevant to Listing \ref{lst:OriginalCode}.}
	\label{fig:RecommendedPost}
	%	\vspace{-.2cm}
\end{figure}
%
In the figure, we only capture the key information 
from the post,~\ie title, question, answer, code and 
display it in the figure. The post contains two 
answers and one of them is useful for the context. 
For instance, the depicted snippet contains class 
\code{CurrencyRoute} where \code{addRoutes()} is 
informative and \code{configure()} is completely 
defined. More importantly, this code shows that 
some additional packages are required, 
\eg~\code{ActiveMQConnectionFactory} 
or~\code{JmsComponent}. In this sense, the 
accompanying snippet is handy for supporting the 
development of the context code in 
Listing~\ref{lst:OriginalCode} since it provides a 
better insight into how to use the related API.
%, which is not the case by 


\smallskip
When the context code shown in Listing 
\ref{lst:OriginalCode} is fed to \FC, the system 
fails to return any results. We anticipate that 
this is due to the lack of input data, \ie the query code is very brief, and to the 
indexing process of \FC, which ignores some 
important components in source code when preparing 
the indexed data. Thus, we believe that there is still room for improvement. In this respect, Lucene 
offers a well-defined platform for managing 
and indexing data. However, it is incumbent upon 
the Lucene user to decide which data to index and 
which data to use as query. To this end, we propose 
an approach to improve the module for searching SO 
posts of \FC. We also attempt to perform various 
refinement steps on the input SO dump as well as to 
%better 
polish the query code. The details of the 
proposed approach are given in the next section.



\subsection{Proposed Approach} \label{sec:SOrec}




Given a user context with code being developed, we aim at searching for posts 
that contain highly relevant answers from StackOverflow. We attempt to 
overcome the limitations of the existing approaches 
by properly indexing SO data and by processing the 
query by developers' side, exploiting various 
refinement techniques. 
%To be concrete, we have the 
%following proposals. 
%To be concrete, we introduce a practical solution that boils down to the following proposals. 
%
%
%We extract the following fields from each post: title, and body, and source code. 
%\subsection{Architecture}
%We impose various measures on the both phases.
%to tokenize. The JDT parser
%
%
In particular, we come up with a comprehensive 
approach named \SR, which takes into consideration 
three consecutive phases,~\ie~Index Creation, Query 
Creation, and Query Execution. By Index Creation, 
we parse and organize an SO dump into a queryable 
format to facilitate future search operations. 
Query Creation is done at the developer's side to 
transform the current context into an informative 
query that can be used to search against the 
indexed data. Concerning Query Execution, the 
actual searching is performed by means of Apache 
Lucene.

Index and query creations rely on the JDT parser, 
which allows one to define different types of 
constructs to be parsed from the source as a 
parameter. In particular, there are the following 
options:%The possible parser options are defined as 
%follows: 

\begin{itemize}
	\item [--] \code{Compilation\_Unit}: the source is parsed as a compilation unit.
	\item [--] \code{Class\_Body\_Declarations}: the source is parsed as a sequence of class body declarations.
	\item [--] \code{Expression}: the source is parsed as a single expression.
	\item [--] \code{Statements}: a constant is used to specify that the source be parsed as a sequence of statements.
\end{itemize}

This list is ordered according to the information that they compute and the severity of the parser option, \eg~the~\code{Compilation\_Unit} option allows one to get more information than the others but it is less resilient to malformed statements.



\begin{figure*}[t!]
	\centering	
	%	\vspace{-.2cm}
	\includegraphics[width=0.99\textwidth]{figs/Architecture.pdf}
	%\vspace{-.3cm}
	\caption{The \SR architecture.}
	\label{fig:SOrecArchitecture}
	%	\vspace{-.4cm}
\end{figure*}

An overview of the \SR building components is 
depicted in Figure~\ref{fig:SOrecArchitecture}. The 
three constituting phases, \ie Index Creation, 
Query Creation, and Query Execution are described 
in detail by the following subsections. 

\subsubsection{Index Creation}\label{sec:Index}

Starting from an SO dump, the original data is loaded into MongoDB for further 
processing. Then, the data is parsed and transformed into a format that can be 
queried later on. At this point, it is necessary to use indexed data for 
future look up. In this work, we opt for Apache Lucene as it is a powerful IR 
tool being widely used to manage and query vector data. For each SO post, the 
following components are excerpted: Title, Body and Code. Concerning the 
textual part, we extract questions, answers, and titles and index them by means 
of the \code{Indexer}. Meanwhile, code contents are parsed to extract useful 
artifacts before being fed to Lucene. In particular, the JDT parser is used to 
obtain six tokens as shown in Table~\ref{tab:Facets}. However, code snippets in 
StackOverflow posts may neither be complete nor compilable~\cite{Sirres2018}, 
and therefore they might not be found if being queried in their original 
format. Thus, to make them compilable, we propose two refinement steps, namely 
\emph{Post cleaning and filtering} and \emph{Code wrapping} as explained below. 

\paragraph{Post cleaning and filtering}\label{sec:cleaning}

In SO messages, a question is typically followed by 
answers and comments. However, many posts do not 
have any answers at all. Such these posts are 
considered not useful for recommendation tasks. 
Thus, we filter out irrelevant posts as well as 
remove the low-quality ones first by considering 
only those that have accepted answers. Then, only 
posts that contain the \code{code} tag\footnote{We 
	are aware that there are SO posts that 
	do not always use the \code{code} tag to include 
	inline 
	source 
	code. Thus, relying only on such a tag might 
	discard messages that instead should be kept. 
	Natural Language Processing techniques can be 
	exploited to make the employed cleaning and 
	filtering phase less strict even though we defer 
	this as future work.} to include in their bodies source code written in Java 
are accepted for further processing. 

\paragraph{Code wrapping}\label{sec:import}% Library import deductions 
%Addition of import directives
%Code reconstruction

%Does FaCoY also apply this? No!

%<<<<<<< HEAD
%Rascal~\cite{5279910} and M3 models~\cite{7070485} help us extract canonical names. 
%Mining class canonical names: In~\cite{DBLP:journals/corr/abs-1901-05392}, the authors propose an approach to mine the Maven central and create a global dependency graph. 

To deal with incomplete and uncompilable snippets, we use the parsing option that yields more tokens. Furthermore, a default class wrapping is added to those snippets that cannot be parsed. For code snippets without any imports, we wrap up with relevant classes to make them more informative. To this end, we exploit an archive provided by \emph{Benelallam~\etal}~\cite{amine_benelallam_2018_1489120}. The dataset contains more than $2.8$M artifacts together with their dependencies as well as other relationships, \eg~versions. We count the frequency that each artifact is invoked, and sort into a ranked list in descending order. Then only top N class canonical names, \ie the ones appear in an import statement, are selected. By parsing all API calls within a method declaration, we trace back to their original packages from the top N names. Nevertheless, given that a class instance is invoked without any declaration, more than one canonical name could be found there. In this case, we compute the Levenshtein distance from each name to the title and body text of the post and use it as a heuristic to extract the best-matched one. Finally, the corresponding import directives are placed at the beginning of the code.


\begin{lstlisting}[caption={Original code snippet.}, label=lst:devContext, 
style=JavaStyle,numbers=left,captionpos=b,xleftmargin=2em,frame=single,framexleftmargin=1.5em]
ASTParser parser = ASTParser.newParser(AST.JLS9);
parser.setResolveBindings(true);
parser.setKind(ASTParser.K_COMPILATION_UNIT);
parser.setSource(snippet.toCharArray());
Hashtable<String,String> options = JavaCore.getOptions();
options.put(JavaCore.COMPILER_DOC_COMMENT_SUPPORT, JavaCore.ENABLED);
parser.setCompilerOptions(options);		
\end{lstlisting}


We consider an example as follows. Listing~\ref{lst:devContext} depicts a code snippet extracted from SO. The code contains just function calls, and it is incomplete since there is no class declaration and import. If we use this code without any refinement to index Lucene, it might not be unearthed by the search engine due to the lack of data. Thus, it is necessary to wrap up and augment it with additional information. By adding class fix and import directives, we obtain a new code snippet as shown in Listing~\ref{lst:AugmentedCode}. The resulted snippet resembles a real hand-written code, which probably facilitates the matching process later on.

\smallskip

\begin{lstlisting}[caption={Augmented code snippet.}, label=lst:AugmentedCode, style=JavaStyle,numbers=left,captionpos=b,xleftmargin=2em,frame=single,framexleftmargin=1.5em]
import java.util.HashMap;
import java.util.Hashtable;	
import org.eclipse.jdt.core.JavaCore;
import org.eclipse.jdt.core.dom.AST;
import org.eclipse.jdt.core.dom.ASTParser;
import org.eclipse.jdt.core.dom.ASTVisitor;	

public class fix(){
  ASTParser parser = ASTParser.newParser(AST.JLS9);
  parser.setResolveBindings(true);
  parser.setKind(ASTParser.K_COMPILATION_UNIT);
  parser.setSource(snippet.toCharArray());
  Hashtable<String, String> options = JavaCore.getOptions();
  options.put(JavaCore.COMPILER_DOC_COMMENT_SUPPORT, JavaCore.ENABLED);
  parser.setCompilerOptions(options);
}	
\end{lstlisting}


Once the refinement steps have been done, we index all terms corresponding to the tokens specified in the  \code{Code} part of Table~\ref{tab:Facets} and store them into Lucene for further look up.


\begin{table}[!h]
	\small
	\centering
%	\vspace{-.3cm}
	%\begin{tabular}{|p{0.3cm}|p{2.4cm}|p{4.8cm}|}\hline
	\begin{tabular}{ p{0.5cm} p{3.5cm} p{8.5cm}}\hline
		\rowcolor{verylightgray}
		& \textbf{Token} & \textbf{Description} \\ \hline
		{\multirow{3}{*}{\rotatebox[origin=c]{90}{Text}}} & \codeS{Title} & The title of the post \\ \cline{2-3}					
		& \codeS{Answer} & All answers contained in the post \\ \cline{2-3}										
		& \codeS{Question} & The question \\ \hline		
		{\multirow{6}{*}{\rotatebox[origin=c]{90}{Code}}} & \codeS{ImportDeclaration} & The directives used to invoke libraries \\ \cline{2-3}					
		& \codeS{MethodDeclaration} & Method declarations with parameters \\ \cline{2-3}					
		& \codeS{MethodInvocation} & API function calls \\ \cline{2-3}					
		& \codeS{VariableType} & Types of all declared variables \\ \cline{2-3}					
		& \codeS{VariableDec} & All declared variables \\ \cline{2-3}										
		& \codeS{ClassInstance} & Class declarations \\ \hline										
	\end{tabular}
	\caption{The used facets.}	
%	\vspace{.2cm}	
	\label{tab:Facets}
\end{table} 




%
%Map<String, String> env = new HashMap<>(); 
%env.put("create", "true");	
%URI uri = URI.create("jar:file:/codeSamples/zipfs/zipfstest.zip");	
%try (FileSystem zipfs = FileSystems.newFileSystem(uri, env)) {
%	Path externalTxtFile = Paths.get("/codeSamples/zipfs/SomeTextFile.txt");
%	Path pathInZipfile = zipfs.getPath("/SomeTextFile.txt");          
%	// copy a file into the zip file
%	Files.copy(externalTxtFile, pathInZipfile, StandardCopyOption.REPLACE_EXISTING); 
%}

%	StringBuilder sb = new StringBuilder();
%	sb.append("Test String");	
%	File f = new File("d:\\test.zip");
%	ZipOutputStream out = new ZipOutputStream(new FileOutputStream(f));
%	ZipEntry e = new ZipEntry("mytext.txt");
%	out.putNextEntry(e);	
%	byte[] data = sb.toString().getBytes();
%	out.write(data, 0, data.length);
%	out.closeEntry();	
%	out.close();

%\subsection{Dataset Creation}
%\subsection{Indexing}



%\subsection{Entropy integration}
%In this section, we describe the mathematical concepts behind the entropy to better understand the context in which we are. Information retrieval is a very large topic in the research community and we focus on this particular technique because it helps us to enhance the provided recommendation. 
%In its general interpretation, the entropy proposed by Shannon 
%\begin{equation}
%H = - \sum p(x) log p(x)
%\end{equation}

%This phase starts with t
%as input for the query creation. The code is parsed 
%The following information is extracted to build a query:
%'s context is the input for the query creation phase
%. The code snippet being developed is parsed using JDT.
%Query: Starting from user's context, we need to build a query.
%is formed by 
%An example is in the following form: ImportDeclaration: org.apache.elasticsearch.indexer; OR MethodDeclaration: get. 
%The idea is to enrich with a MAIN  improvement: boosting. 
%that the developer is working on, we parse 
%tell to Lucene that an index is more important with respect to another
%. Boosting is the mechanism to
%The original code is parsed to get all the import directives. 
%Given a code snippet,
% and we propose

\subsubsection{Query Creation}

%A flat query is the one that treats all terms equally. 
%Together with six tokens emerging from source code, there 
%To build tokens to match against the Title, Answer, and Question tokens which are shown in the first half of Table~\ref{tab:Facets}, 


This phase is conducted on the client side, and the 
method declaration being 
developed is used as input context. A query can be 
formed by considering all 
terms extracted from the context code. It is 
evident that each term in posts 
has a different level of importance. Thus, the 
second phase is to equip a query 
with more information that better describes the 
current context, taking into 
account the terms' importance level. Fortunately, 
Lucene supports 
\emph{boosting}, a scoring mechanism to assign a 
weight to each indexed token. 
Based on scoring, we perform two augmentation 
steps,~\ie~\emph{Boosting}, and 
\emph{Tokenizing} as follows.

% stored in Lucene,



\paragraph{Boosting}\label{sec:boosting}
The original code is parsed to obtain the six tokens listed in the last half of Table~\ref{tab:Facets}. Each term in the code is assigned a concrete weight to boost the level of importance. Entropy~\cite{DBLP:journals/sigmobile/Shannon01} is exploited to compute the quantity of information of a document using the following formula: 

\begin{equation}
H = - \sum p(x) log p(x)
\end{equation} 

where $p(x)$ is the probability of term $x$. An entropy value ranges from $0$ to $log(n)$, where $n$ is the number of terms within the document. We compute entropy for all terms in the original source code and rank them in a list of descending order. Then the first quarter of the list is assigned a boost value of $4$. Similarly, the next $2^{nd}$, $3^{rd}$, and $4^{th}$ quarters get the boost value of $3$, $2$, and $1$, respectively. Finally, all the code terms are attached to their corresponding tokens to form the query.



%Each term is assigned a boost score as follows. 

\paragraph{Tokenizing}\label{sec:tokenizing}
By the Index Creation phase in Section~\ref{sec:Index}, nine different tokens 
have been populated (see Table~\ref{tab:Facets}). Among them, there are $3$ 
textual tokens, \ie Title, Answer, and Question. However, by the developer's 
side, the input context contains just source code and there are no textual 
parts that can be used to match against the three tokens. Thus, given the input 
code, we attempt to generate textual tokens by exploiting the import directives 
embedded at the beginning of each source file. Starting from an import 
directive, we break it into smaller pieces and attach them to all the textual 
tokens. A previous work~\cite{Borg:2014:RSD:2652524.2652556} shows that in an 
SO post, the title is more important than the description. In particular, 
according to~\cite{Borg:2014:RSD:2652524.2652556} the importance ratio between 
description and title of a given post is $1/3$. Accordingly, we 
set a boost value of $4$ to the title and $1.4$ to both the answer and 
question. 

\smallskip
By considering the code in Listing~\ref{lst:OriginalCode}, the query that \SR creates after the boosting and tokenizing phases is shown in Listing~\ref{lst:Token}.%ready to be executed 

%Take as an example, given the import directive 
%\code{org.apache.camel.CamelContext} from the code in 
%Listing~\ref{lst:OriginalCode}, then it is tokenized and transformed into a 
%partial query as shown in Listing~\ref{lst:Token}.

%org.apache.elasticsearch.indexer
%Title: apache OR Title: elasticsearch OR Question: apache OR Question.

%\begin{lstlisting}[caption={A partial query produced from an import 
%directive}, label=lst:Token, style=NormalStyle]
%
%Title=apache^4 OR Title=camel^4 OR Answer=apache^1.4 OR Answer=camel^1.4 OR 
%Question=apache^1.4 OR Question=camel^1.4
%\end{lstlisting}

\begin{lstlisting}[caption={Sample query produced after the \textit{Boosting} and \textit{Tokenizing} phases.},label=lst:Token, captionpos=t,language=SOrec,numbers=none]
VariableDeclarationType: CamelContext^1.0 OR 
VariableDeclaration: context^1.0 OR 
MethodInvocation: addRoutes^1.0 OR 
ClassInstance: DefaultCamelContext^1.0 OR 
ImportDeclaration: org.apache.camel.impl.DefaultCamelContext^1.0 OR 
ImportDeclaration: org.apache.camel.CamelContext^1.0 OR 
ClassInstance: RouteBuilder^1.0 OR
MethodDeclaration: main^1.0 OR 
ImportDeclaration: org.apache.camel.builder.RouteBuilder^1.0 OR 
MethodDeclaration: configure^1.0 OR 
Answer: apache^1.4 OR 
Answer: camel^1.4 OR 
Question: apache^1.4 OR 
Question: camel^1.4 OR 
Title: apache^4 OR 
Title: camel^4
\end{lstlisting}


\subsubsection{Query Execution} \label{sec:QueryExecution}


%\subsubsection{Ranking}\label{sec:ranking}

%Code in StackOverflow posts may. 
%We have done this comparison, based on the 
%empirical results because this 
%topic reaches higher relevance in the research 
%community. 
%Moreover, we describe the differences between two 
%Lucene ranking methods, the 
%Best Matching 25 (BM25) 
%\cite{Robertson:2009:PRF:1704809.1704810} and the 
%classical term frequency-inverse document 
%frequency (TF-IDF).
%\PN{@Riccardo: please add more descriptions for 
%this part. It is unclear to 
%me.}

%The term frequency-inverse document frequency 
%(TF-IDF) considers the relevance 
%of a term by tanking into account its frequency 
%within a document. It 
%increases 
%the score proportionally to the number of times a 
%word appears in the document 
%and is offset by the number of documents in the 
%corpus that contain the word, 
%which helps to adjust for the fact that some words 
%appear more frequently in 
%general. 

%=============from FaCoY paper: Our approach 
%computes rankings of the search 
%results based on a scoring function that measures 
%the similarity between the 
%code query and matched code snippets.

%Lucene embedded implementation of this,
%Going beyond the theoretical aspects, we choose to 
%use the Lucene BM25 
%implementation because it is better than TF-IDF 
%from empirical experiment that 
%we will show in the \Cref{sec:Evaluation}.
%The Equation \ref{eqn:BM25} describes this ranking 
%function:

Queries that are created, as described in the 
previous section, are executed by means of Apache 
Lucene. Moreover, we exploit the Lucene built-in 
BM25 to rank indexed posts. In particular, BM25 is 
a bag-of-words retrieval 
function that ranks a set of documents based 
on the query terms appearing in each document, 
regardless of the inter-relationship between the 
query terms within a document, \eg their 
relative proximity. The index is computed as given 
below.

\vspace{-.3cm}
\begin{equation} \label{eqn:BM25}
R (q,d) = \sum_{t \in q} \frac{ f_t^d} {k_1((1-b) + 
	b \frac{l_d}{avgl_d} + 
	f_t^d} 
\end{equation}
%\vspace{-.2cm}
where $f_t^d$ is the frequency of term $t$ in 
document $d$; $ l_d $ is the 
document d length; $avgl_d$ is the document average 
length along the 
collection; $k$ is a free parameter usually set to 
$2$ and $b \in [0,1]$. When 
$b=0$, the normalization process is not considered 
and thus the document length 
does not affect the final score. In constrast, when 
$b=1$, the full-length 
normalization is performed. In practice, $b$ is 
normally set to $0.75$. It has 
been shown that for ranking documents, BM25 works 
better than the standard 
TF-IDF one~\cite{DBLP:journals/corr/abs-0911-5046}. 

%the BM25 is the. 

By considering the query in Listing \ref{lst:Token} 
as input, the post shown in Figure~\ref{fig:RecommendedPost} is among the 
resulting ones.

\smallskip
In the following section we introduce two 
evaluations to examine if our proposed solution is 
beneficial to the matching of relevant SO posts.	







\subsection{Evaluation} \label{sec:SOrecEvaluation}


To study \SR's performance, we performed two main evaluations by means of user 
studies. The first one is done to evaluate the role of each augmentation 
proposed in Section~\ref{sec:SOrec}. To this end, we consider $6$ 
experimental configurations,~\ie $\textbf{A}, \textbf{B}, \textbf{C}, 
\textbf{D}, \textbf{E}, \textbf{F}$ with $10$ queries for each (see 
Table~\ref{tab:TestConfigurations}). The second evaluation compares \SR against 
a baseline, namely the module for retrieving SO posts of 
\FC~\cite{DBLP:conf/icse/KimKBC0KT18}, and this corresponds to the last 
configuration $\textbf{G}$. For the sake of representation, from now on the 
baseline is addressed as \FC (unless otherwise stated), despite the fact that 
it is only a module of the whole \FC system presented 
in~\cite{DBLP:conf/icse/KimKBC0KT18}. To thoroughly examine the difference in 
their performance, we consider $50$ queries in $\textbf{G}$. The queries 
contain code snippets that invoke ten of the most popular Java libraries,~\ie 
Jackson, SWT, MongoDB driver, Javax Servlet, JDBC API, JDT core, Apache Camel, 
Apache Wicket, Twitter4j, Apache POI. 

The test configurations are explained in Table~\ref{tab:TestConfigurations}, 
whose the $2^{nd}$ to $5^{th}$ columns specify the presence of the techniques 
mentioned in Section~\ref{sec:SOrec}, with the corresponding section 
being shown in parentheses. For example, the $2^{nd}$ column~\textbf{Wrapping} 
is a combination of \emph{class fixing} and \emph{library import deduction} 
introduced in Section~\ref{sec:Index}. To facilitate future research, we made 
available the \SR tool together with related data in 
GitHub.\footnote{\url{https://github.com/ase2019-sorec/SOrec}}


\input{src/SOrecEvaluation}

\subsubsection{Dataset}\label{sec:SOrecDataset}
%According to the Stack Exchange data counter\footnote{\url{https://stackoverflow.com/questions/tagged/java}}, 
To provide input for the evaluation, we %first downloaded the newest 
exploited a recent 
StackOverflow dump\footnote{\url{https://archive.org/details/stackexchange}}
%(as of March 2019)
which is an XML file of 70GB in size and contains more than 
$18$ millions posts. By filtering with tags, we obtained $757,439$ posts 
containing Java source code. The resulting set has more than $1,2$ millions of 
answers with $49.20\%$ of them being already accepted \ie~$552,458$ answers. 
In such posts there were $32,578$ snippets that did not have any imports. We 
fixed them as presented in Section~\ref{sec:import}. Eventually, we indexed 
and parsed all the posts following the paradigm described in 
Section~\ref{sec:Index}. More details of the dataset used in our evaluation are 
shown in Table~\ref{tab:Datasets}.

\subsubsection{User studies} \label{sec:Methodology}
%User study 
%It is necessary to evaluate how relevant the projects are, compared to the query project. Since user study is the only way to evaluate the outcome \cite{McMillan:2012:DSS:2337223.2337267,10.1109/SANER.2017.7884605}, we involved a group of $10$ software developers to participate in the manual evaluation. 
%To get information about the participants related to their development background, we sent them a questionnaire. 
%Furthermore, their favorite code platform is StackOverflow, where they normally search for posts that are useful for their current development tasks. 
%To evaluate the performance, 

We resort to user study as this is the only way to investigate whether the recommendation outcomes are really helpful to solve a specific task~\cite{Lo:2012:DSA:2473496.2473616,McMillan:2012:DSS:2337223.2337267,DBLP:journals/ese/PonzanelliBPOL16}. A group of $11$ developers was asked to participate in the user study. Six participants are master students attending a Software Engineering course. Three of them are PhD students. The other two are postdoc researchers. Through a survey sent to each participant, we found out that more than a half of them have at least $7$ years of programming experience. Among these people, three participants have worked with programming for $15$ years. All of them are capable of Java and at least another programming language, \eg Python or C++. The evaluators use code search engines like GitHub, StackOverflow, or Maven on a daily basis. Furthermore, they frequently re-use code fragments collected from these external sources.% quite often.

The user studies aim at evaluating the relevance of a recommended post and a 
code snippet. Given a query, each system, \ie \FC or \SR produces as outcome in the form a 
ranked list of relevant posts. To aim for a fair evaluation, we mixed the 
top-$5$ results generated by each system in a single Google form and present 
them to the evaluators together with the corresponding context code. This 
simulates a \emph{taste test}~\cite{Ghose2001,doi:10.1108/13522750810879048} 
where users are asked to give feedback for a product, \eg~food or drink, 
without having a priori knowledge about what is being addressed. This aims to 
eliminate any bias or prejudice against a specific system. Each pair of code 
and post, \ie $<$\textit{query, retrieved post}$>$ is examined and evaluated by 
at least two participants using the scores listed in Table~\ref{tab:Scores}. 
Apart from $11$ developers mentioned before, we also involved one more senior 
researcher to validate the evaluation outcome of every query. In case there 
is a disagreement between any two participants, \eg the first person assigned 
the score of $2$ and the second one gave $4$ to a same pair, the senior 
researcher examines the pair again to eventually reach a consensus.%and reach 
%the final decision.  and discuss 

%and afterwards double-checked by a third person to fix any possible discrepancies.
\vspace{.3cm}		






\subsubsection{Evaluation metrics} \label{sec:Metrics}
As typically done in related work, the following metrics have been considered to evaluate the recommendation outcomes~\cite{Lo:2012:DSA:2473496.2473616,McMillan:2012:DSS:2337223.2337267}:
%of a system with respect to the user study

\begin{itemize}
	\item \textit{Confidence}: it is the score given to a pair of $<$\textit{query, retrieved post}$>$ following Table~\ref{tab:Scores}; %the confidence of an evaluator is the score she assigns to the similarity between the projects;
	\item \textit{Success rate}: if at least one of the top-5 retrieved posts receives $3$ or $4$ as score, the query is considered to be relevant. {\em Success rate} is the ratio of relevant queries to the total number of queries;
	\item \textit{Precision}: it is computed as the ratio of pairs in the top-$5$ list that have a score of $3$ or $4$ to the total number of pairs, \ie $5$.% pairs.% labelled as \code{Similar} or \code{Highly similar} by humans. 
\end{itemize}

%Further than the previous metrics, we introduce an additional one to measure the ranking produced by the similarity tools. For a query, a similarity tool is deemed to be good if all top-5 retrieved projects are relevant. In case there are false positives, \ie those that are labeled \codeS{Dissimilar} and \codeS{Neutral}, it is expected that these will be ranked lower than the true positives. In case an irrelevant project has a higher rank than that of a relevant project, we suppose that the similarity tool is generating an improper recommendation. The \emph{Ranking} metric presented below is a means to evaluate whether a similarity metric produces properly ranked recommendations.%, which are properly ranked. 

%We express in another way.
%Notice that the CFPRS involves the creation of the indexes, so the results are the same with respect the CRFLT in term of scoring and recommended item. To show the changes in an effective way, we consider both the manual scoring, given following the Table \ref{tab:Scores}, and our scoring system that considers all the mentioned features. In particular, we consider the delta from one configuration to another: in this way, we can rank the different configurations considering the degree of enhancement in the query.
%We compared directly with the SO module of \FC. 

\subsubsection{Research questions}  \label{sec:Questions}

The evaluations are conducted to answer the following research questions:

\begin{itemize}
	
	\item \rqfourth We compare the flat configuration with the augmented ones to see which setting fosters the best recommendation outcome for \SR. %This research question attests the contribution of the entropy in the query building. In particular, we will show that this mathematical concept leverages more accuracy and precision in term of recommended snippets with respect to a standard query, \ie without any boosting.
	%	if they really contribute to improvement. This aims at investigating 
	
	\item \rqfifth Compared to \FC, \SR is equipped with various refinement techniques. By answering this question, we ascertain whether our proposed augmentations are useful for searching posts in comparison to the original approach \FC.%With this question, we investigate the differences between the two Lucene weight scheme, the traditional TF-IDF and the BM-25. We evaluate the results using the same context files in order to show that BM-25 performs better than the TF-IDF. We analyze this issue because it is very relevant in  the research community
	
	\item \rqsixth We are interested in understanding the factors that add up 
	to the performance difference between the two systems.%investigate.%Going 
	%%beyond the internal evaluation, we perform a comparison with \FC, another 
	%%tool that exploits the SO posts to perform code recommendations. We 
	%%conduct 
	%%a manual user study, by evaluating the quality of the recommended posts 
	%%against the developer's context.
\end{itemize}

The following section analyzes the systems' performance by addressing these research questions.



\subsection{Experimental Results} \label{sec:SOrecResults}




This section presents the results obtained from the experiments as well as 
related discussions. %In Section~\ref{sec:Analysis}, 
First, we analyze the outcomes 
obtained by performing \SR with six configurations, \ie $\textbf{A} \div 
\textbf{F}$ (see Table~\ref{tab:TestConfigurations}), to answer 
\textbf{RQ$_4$}. Afterwards, we compare \FC with \SR by answering 
\textbf{RQ$_5$}. Finally, we attempt to reason what constitutes the performance 
differences between the two systems by means of \textbf{RQ$_6$}. 
%Threats to validity of the performed experiments are discussed in Section~\ref{sec:SOrecThreats}. %using $\textbf{G}$ 

%\subsubsection{Result Analysis} \label{sec:Analysis}

\noindent \rqfourth


Each configuration is evaluated using $10$ queries and each of them corresponds to $5$ posts, resulting in $50$ pairs of $<$\textit{query, retrieved post}$>$. We gather the confidence scores of each configuration and represent them in a violin boxplot as shown in Figure~\ref{fig:Evaluation1}. According to \emph{Hintze \etal}~\cite{doi:10.1080/00031305.1998.10480559}, a violin boxplot is a combination of boxplot and density traces which gives a more informative indication of the distribution's shape, or the magnitude of the density. Thus, it is evident that performing \SR with flat queries, \ie configuration \textbf{A}, yields the worst performance since the corresponding boxplot is slim and distributed along the vertical axis. This suggests that feeding queries without incorporating any proposed augmentations brings less relevant posts. Meanwhile, the system obtains a better performance for configurations \textbf{B} (flat query plus wrapping) and \textbf{C} (flat query plus wrapping and ranking) with respect to~\textbf{A}. Moreover, the two configurations \textbf{B}, \textbf{C} contribute to a comparable performance as their corresponding violins have a similar shape. Among others, the best confidence is seen when running \SR with \textbf{F}, \ie~all proposed augmentations are incorporated. In particular, no query pair gets $1$ as the confidence value and most of them are assigned a value of $3$ or $4$. This necessarily means that augmenting queries with all the proposed measures helps retrieve highly relevant posts.



	\begin{figure}[t!]
	\centering	
	\includegraphics[width=0.35\textwidth]{figs/Evaluation1.pdf}
	\caption{Confidence for configurations $\textbf{A} \div \textbf{F}$.}
	\label{fig:Evaluation1}
	\end{figure}	



%	\begin{figure*}[t!]
%		\begin{tabular}{c c c c}	
%			\centering    
%			\subfigure[Precision (40 queries)]{\label{fig:PrecisionFaCoYSOrec40}\includegraphics[width=0.45\textwidth]{figs/Precision_FaCoY_SOrec_40.pdf}} &
%			\subfigure[Success rate (40 queries)]{\label{fig:SuccessRateFaCoYSOrec40}\includegraphics[width=0.45\textwidth]{figs/SuccessRate_FaCoY_SOrec_40.pdf}} 
%		\end{tabular}
%		\label{fig:PRF2}
%		\caption{Precision, and success rate for Configuration $\textbf{G}$.}
%	\end{figure*}
	
	



\begin{table}[h!]
	%	\footnotesize
%	\vspace{-.3cm}
	\centering
	\begin{tabular}{lcccccc}
		\toprule
		\multirow{2}[3]{*}{\textbf{Metric}} & \multicolumn{6}{c}{\textbf{Configuration}} \\
		\cmidrule[\lightrulewidth](l){2-7}
		& \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} & \textbf{E}  & \textbf{F} \\
		\midrule	
		Success rate  &  0.90  &  0.90  &  0.90  &  0.90 &  1.00 &  1.00 \\
		Precision   &  0.60  &  0.66  &  0.68  &  0.74 &  0.78 &  0.82 \\
		\bottomrule
	\end{tabular}
	\caption{Success rate and Precision.}
	\label{tab:Precision}
\end{table}


We consider the success rate and precision scores for the configurations in 
Table~\ref{tab:Precision}. Running \SR on the dataset always gets a minimum 
success rate of $0.90$, regardless of the configuration. \SR gains the maximum 
score, \ie $success \quad rate=1$ when \textbf{E} or \textbf{F} is imposed. 
This demonstrates that Tokenizing (see Section~\ref{sec:tokenizing}) 
contributes much to the matching of relevant posts. Concerning 
\emph{Precision}, we see that using flat query obtains the lowest precision, 
\ie $Precision=0.6$ and this is consistent with \emph{Confidence} in Figure 
\ref{fig:Evaluation1}. Again, the best \emph{Precision}, \ie $0.82$ is obtained 
when all augmentations are imposed on the queries. 

%only wrapping (\textbf{A})

\begin{tcolorbox}[boxrule=0.86pt,left=0.3em, right=0.3em,top=0.1em, bottom=0.05em]%
	In summary, running \SR by deploying all proposed augmentations provides 
	the best performance with respect to confidence, success rate, and 
	precision. % There is no distinct 
	%winner between n-gram and bi-gram when they are used to parse input 
	%metamodels. Furthermore, a feature set with more terms is beneficial to 
	%the 
	%prediction outcome
\end{tcolorbox}




%\subsection{Comparison with \FC} \label{sec:ComparisonFaCoY}
%Meanwhile, \FC . 
%than \FC 
%For the example, . We attempt to ascertain why \FC fails in this case. First, the code is very brief and thus it cannot.
% retrieve any single result for the same code query




\medskip
\noindent \rqfifth

To aim for a reliable comparison, we executed both \FC and \SR on the dataset mentioned in~\Cref{sec:SOrecDataset}. Considering the set of $50$ queries, \SR returns $250$ pairs of query-post. Each pair gets a score ranging from $1$ to $4$. However, \FC does not find any results for $10$ among the queries, \ie the corresponding scores are $0$ (see Table~\ref{tab:Scores}). We depict the confidence scores of both systems using violin boxplots in Figure~\ref{fig:ConfidenceFaCoYSOrec50}. The boxplots demonstrate that \SR gains considerably better confidence than that of \FC. In particular, \SR has more scores of $3$ and $4$, whereas \FC has more scores of $1$ and $2$. By inspecting the ten queries that yield no results, we found out that their input context code is considerably short. This supports our hypothesis in Section~\ref{sec:SOrecBackground} that \FC is less effective given that input data is incomplete or missing. %An analysis on the correlation between the number of lines of code and confidence reveals that.


	
\begin{figure*}[t!]
	\begin{tabular}{c c c c}	
		\centering    
		\subfigure[Confidence (50 queries)]{\label{fig:ConfidenceFaCoYSOrec50}\includegraphics[width=0.22\textwidth]{figs/Confidence_FaCoY_SOrec_50.pdf}} & 	
		\subfigure[Confidence (40 queries)]{\label{fig:ConfidenceFaCoYSOrec40}\includegraphics[width=0.22\textwidth]{figs/Confidence_FaCoY_SOrec_40.pdf}} &
		\subfigure[Precision (40 queries)]{\label{fig:PrecisionFaCoYSOrec40}\includegraphics[width=0.22\textwidth]{figs/Precision_FaCoY_SOrec_40.pdf}} &
		\subfigure[Success rate (40 queries)]{\label{fig:SuccessRateFaCoYSOrec40}\includegraphics[width=0.22\textwidth]{figs/SuccessRate_FaCoY_SOrec_40.pdf}} 
	\end{tabular}
	\label{fig:PRF1}
	\caption{Confidence, precision, and success rate for Configuration $\textbf{G}$.}
\end{figure*}


To aim for a more reliable comparison, we remove the ten queries from the results of both systems and sketch the confidence scores in Figure~\ref{fig:ConfidenceFaCoYSOrec40}. For this set of queries, the \FC's violin fluctuates starting from $3$ down to $1$. In contrast, the majority of the violin representing \SR lies on the upper part of the figure, starting from $3$ in the vertical axis. We conclude that \SR obtains a better confidence compared to \FC.

We further investigate the systems by considering Figure~\ref{fig:PrecisionFaCoYSOrec40} where the precision scores for $40$ queries are depicted. By this metric, the performance difference between the two systems becomes more noticeable. To be more concrete, a larger part of the \FC's boxplot resides under the median horizontal line, implying that most of the queries get a precision lower than $0.5$. In the opposite side, \SR gains better precisions that are larger than $0.5$, and agglomerate to the upper bound, \ie~$1.0$. The metric shows that, given the same query, \SR returns more relevant posts than the baseline does.% to the query.


The obtained success rates for both systems are shown in Figure~\ref{fig:SuccessRateFaCoYSOrec40}. Among $40$ queries fed to \FC, $78\%$ of them are successful, \ie at least one pair of a query gets a value of $3$ or $4$. Meanwhile, \SR achieves a better percentage of success, $38$ among $40$ queries are successful, yielding a success rate of $95\%$.

Finally, it is important to understand if the performance difference is 
statistically significant. We compute Wilcoxon rank sum test 
\cite{Wilcoxon1992} 
on the scores 
obtained by the systems and get the following results: p-value for Confidence 
is \emph{1.08e-10}; p-value for Precision is \emph{8.90e-06}; p-value for 
Success rate is \emph{2.00e-02}. The null hypothesis is that there are no 
differences between the performance of \FC and that of \SR. Using $95\%$ as the 
significance level, or p-value $<$ $0.05$ we see that by all quality indicators 
the p-values are always lower than \emph{5e-02}. Thus, we reject the null 
hypothesis and conclude that the performance improvement obtained by \SR is 
statistically significant.


\begin{tcolorbox}[boxrule=0.86pt,left=0.3em, right=0.3em,top=0.1em, bottom=0.05em]%
	\SR outperforms \FC in terms of confidence, success rate, and precision. 
	Furthermore, the performance difference between the two systems is 
	statistically significant.
\end{tcolorbox}


\medskip
\noindent \rqsixth

%We in 
%Before analyzing the two systems' performance, w
We refer back to the example introduced in~\Cref{sec:SOrecBackground}. Actually, the post in Figure~\ref{fig:RecommendedPost} is recommended by \SR when the code in Listing~\ref{lst:OriginalCode} is used as query. In this example, compared to the baseline, \SR works better since it is capable of recommending a very relevant and helpful discussion, while it is not the case with \FC. By carefully investigating the query generated by \SR, we see that the transformation of import directives to produce textual tokens as shown in Listing~\ref{lst:Token} is beneficial to the search process: it equips the query with important terms which then match with the post's title. Table~\ref{tab:Comparison} distinguishes between the two systems by listing the facets exploited by each of them.

\begin{table}[h!]
	\small
	\centering
	\begin{tabular}{lcc} \hline	
		%		\toprule			
		\rowcolor{verylightgray}
		{\bf Technique} & {\bf \FC} & {\bf \SR} \\  \hline		
		Code analysis & \cmark  & \cmark \\  \hline
		Class fixing & \cmark &  \cmark \\\hline
		%		Lucene Index & $\times$ & $\times$ \\  \hline
		Import mining & --- & \cmark \\  \hline		
		Entropy & --- &  \cmark \\\hline		
		BM25 & --- & \cmark \\\hline				
		Tokenizing & --- & \cmark \\\hline				
		%		\bottomrule
	\end{tabular}
	\caption[Experimental configurations]{Comparsion between \FC and \SR.}
	\label{tab:Comparison}
\end{table}

%Meanwhile \SR exploits the boosting feature. 
%Moreover, \FC uses TF-IDF as the ranking scheme that is outperformed by the BM-25 technique. 

\FC exploits the Porter stemming algorithm and the English analyzing utilities 
provided by Lucene to perform a query. It parses the developer's source code as 
well as comments and uses extracted indexes described in~\Cref{sec:SOrecBackground} 
to search. As shown in \textbf{RQ$_4$} and \textbf{RQ$_5$}, a flat query 
containing only full-text is not sufficient to retrieve useful results. Though 
\FC employs Lucene as its indexer, it does not exhaustively exploit boosting 
which is considered to be the heart of Lucene. To this end, \SR attempts to 
improve the baseline by imposing various boosting measures. By the Index 
Creation phase, \SR enriches incomplete code snippet with class and import 
directives and then tokenizes them. By the Query Creation and Execution phases, 
\SR exploits import directives from source code to build indexes to match 
against indexed textual data. Since \FC does not perform these phases, it is 
unable to match source code with textual context in post. Furthermore, \FC 
cannot match input code with snippets stored in database but without import 
directives. %In this sense, we see that \SR is able to. Moreover, \SR uses 
%different tokens in the searching phase with respect to \FC and this may 
%affect 
%the final results in term of the quality of retrieved posts. 

%We pay more attention to. 
% to match against the 
%Although we consider only the Facoy query module, it clearly affects final results coming from GitHub. About the missing results, we select randomly contexts from Github, so these failures may do to the context length or missing information. 
%, as it performs only a query based on text analysis

\begin{tcolorbox}[boxrule=0.86pt,left=0.3em, right=0.3em,top=0.1em, bottom=0.05em]
	Altogether, the query boosting scheme and the considered facets for 
	the creation of indexes are attributed to the performance difference 
	between the two systems. %, which is not fully exploited in \FC
\end{tcolorbox}



\subsection{Threats to validity} \label{sec:SOrecThreats}

We investigate the threats that may affect the validity of the experiments as well as the efforts made to minimize them. %In particular, we focus on internal and external threats to validity as discussed below. We identify both internal and external threats that may

\smallskip
\noindent
\textit{\textbf{Internal validity.}} It concerns any confounding 
factors that may have an influence on our results. We 
attempted to avoid any bias in the user studies by: 
\emph{(i)} involving $11$ developers with different 
levels of programming experience; \emph{(ii)} 
simulating a taste test where users are not aware of 
what they are evaluating. Furthermore, the labeling 
results by two evaluators were then double-checked by 
another senior researcher to aim for soundness of the 
outcomes.%; (\emph{ii}) by completely 
%automating the evaluation of the defined metrics 
%without any manual intervention. Indeed, the 
%implemented tools could be defective. To contrast and 
%mitigate this threat, we have run several manual 
%assessments and counter-checks.

\smallskip
\noindent
\textit{\textbf{External validity.}} This refers to the generalizability of the obtained results and findings. To contrast and mitigate this threat, we enforced the following measures. The sets of code snippets that have been selected as queries invoke various Java libraries. Furthermore, the number of code lines of the queries ranges 
from $22$ to $608$, attempting to cover a wide range of 
possibilities in practice. Our approach is also applicable to other programming languages, however, in the scope of this work we restricted ourselves to perform evaluations on posts containing Java source code.

\smallskip
\noindent
\textit{\textbf{Construct validity.}} This is related to the experimental settings used to evaluate the similarity approaches. We addressed the issue seriously and attempted to simulate a real deployment scenario where the tools are used to search for relevant posts from StackOverflow. In this way, we were able to investigate if the tools are really applicable to authentic usage.

%measurement of. the. measured only the. 

\smallskip
\noindent
\textit{\textbf{Conclusion validity.}} This is whether the exploited experiment methodology is intrinsically related to the obtained outcome, or there are also other factors that have an impact on it. The evaluation metrics, \ie Success rate, Confidence, Precision  might cause a threat to conclusion validity. To confront the issue, we employed the same metrics to evaluate both \FC and \SR.



==> src/SOrecEvaluation.tex <==
\begin{landscape}
\begin{table*}[t!]
	\vspace{2.0cm}
	\footnotesize
	\centering
	\begin{tabular}{cccccc p{10.2cm}}  \hline	
		\rowcolor{verylightgray}	
		{\multirow{2}{*}{\bf Conf.}} & \textbf{Wrapping}  & 
		\textbf{ Boosting} & \textbf{Tokenizing} & \textbf{ Ranking} & 
		{\multirow{2}{*}{\bf \# of queries}} & {\multirow{2}{*}{\bf Description}} \\ 
		& (Sec.~\ref{sec:Index})  & 		(Sec.~\ref{sec:boosting}) & (Sec.~\ref{sec:tokenizing}) & (Sec.~\ref{sec:QueryExecution}) &  &   \\  \hline		
		\textbf{A} & --- & --- & --- & --- & $10$ & Flat queries, without 
		considering any proposed augmentations \\ \hline 
		\textbf{B} & \cmark & --- & --- & --- & $10$ & Wrapping is introduced to queries in Conf. A \\\hline
		\textbf{C} & \cmark & --- & --- & \cmark & $10$ & BM25 is used to rank the retrieved posts \\\hline
		\textbf{D} & \cmark  & \cmark & --- & ---& $10$ & Entropy is used to boost the queries in Conf. B \\\hline
		\textbf{E} & \cmark  & --- & \cmark & --- & $10$ & Transforming import directives to textual tokens for queries in Conf. B \\\hline		
		\textbf{F} & \cmark & \cmark & \cmark & \cmark & $10$ & Imposing all proposed augmentations   \\\hline
		\textbf{G} & \cmark& \cmark& \cmark & \cmark & $50$ & Imposing all 
		proposed augmentations to compare \SR and \FC 
		\\\hline		
	\end{tabular}
	\caption[Experimental configurations]{Experimental configurations.}
	\label{tab:TestConfigurations}
\end{table*}

\begin{table}[h!]
	\footnotesize
	\centering
	\begin{tabular}{ll|ll}  \hline	
		\rowcolor{verylightgray}	
		{\bf Name} & {\bf Value} & {\bf Name} & {\bf Value} \\ \hline		
		{\bf Size} & $70$GB & {\bf \# of answers} &  $1,122,789$ \\ \hline		
		{\bf \# of posts} & $18,300,672$ & {\bf \# of acc. answers} & $552,458$ 
		\\ \hline		 
		{\bf \# of Java posts} & $757,439$ & {\bf \# of posts fixed} & $32,578$ 
		\\ \hline		
	\end{tabular}
	\caption[Statistics]{A summary of the SO dump used in the evaluation.}
	\label{tab:Datasets}
\end{table}

\begin{table}[h!]
	\footnotesize
	\centering
%	\vspace{-.2cm}

	\begin{tabular}{r p{11.0cm}} \hline	%p{0.25\linewidth}		
		\rowcolor{verylightgray}
		%		\toprule
		\textbf{Score} & \textbf{Description} \\ \hline
		%		\midrule		
		0 & No results at all are returned \\ \hline
		1 & The post is totally irrelevant \\ \hline %/The snippet contains help to the developer
		2 & The post contains some hints but it is still out of context \\ \hline
		3 & There are relevant suggestions but the key features are missing \\ \hline
		4 & The post provides proper recommendations, together with its code snippets it can help developers solve their current task \\ \hline					
		%		\midrule
		%		& \textbf{Total} & \textbf{555} \\ %& \textbf{--,--}
	\end{tabular}
	\caption{Confidence Scores.}
%	\vspace{-.3cm}
	\label{tab:Scores}
\end{table}
\end{landscape}

==> src/aethereal.tex <==
%In this section, w

In~\Cref{sec:aethereal}, we present \aethereal, our prototype tool for cross-projects migration dependencies graph definition. Afterwards, we introduce some interesting use cases of migration graphs in Section~\ref{sec:aethereal-result}.
\begin{figure}
	\centering
	\includegraphics[width=0.80\linewidth]{figs/migration-graph}
	\caption{Cross-project migration dependencies.}
	\label{fig:migration-graph}
\end{figure}

\subsubsection{\aethereal}\label{sec:aethereal}
%The nodes are 3rth part libraries. 
%In particular, given two versions of a library, (\ie~Lib\_v1 and Lib\_v2) a specific CPMDG is built. It allows to extract all the clients that migrate from an initial version of the library to an updated one.

Figure~\ref{fig:migration-graph} depicts a snapshot of a cross-projects migration dependencies graph (CPMDG). We distinguish between clients and libraries as follows. Third-party libraries are blank nodes and they identify the versions that should be migrated, whereas clients (grey nodes) are dependencies that use the libraries. The edges between can be \emph{(i)} usage dependencies which are depicted as grey solid edges between a library and a client, or \emph{(ii)} version dependencies, which are dotted edges among libraries. \aethereal is a tool written in Java that aims at supporting the automatic generation of CPMDG. The current version of \aethereal is both available online\footnote{\url{https://github.com/ crossminer/aethereal}} and fully integrated into the KB. Maven-miner\footnote{\url{https://github.com/diverse-project/maven-miner}} tool extracts the Maven Dependency Graph, which is a graph-based representation of the Maven Central Repository\footnote{\url{https://search.maven.org/}}~\cite{amine_benelallam_2018_1489120}. A graph snapshot has been showcased in~\cite{DBLP:journals/corr/abs-1901-05392}. \aethereal uses the Maven-miner dataset to compute the library CPMDGs and provides three different mining modes as follows:

\begin{itemize}
	\item Client usage identification: given a specific library version, it provides the list of clients that use the library version.
	\item Migrated client pairs: given two versions of a library, it computes all the clients that have been already migrated from the initial version to the evolved one. This information is useful to understand how other clients deal with the migration of library breaking changes. Table~\ref{tab:client-pairs} reports a simple client pairs result.
	\item Dependency version matrix: given a library without any version, \aethereal computes a dependency matrix where each column corresponds to a library version, each row is a non-version client; each cell contains the client version that uses the specific library version. A sample of the dependency version matrix is reported in Table~\ref{tab:dependency-version-matrix}. Moreover, the  migrated client pairs are computed for each library version pairs.
\end{itemize}


\begin{table}[h!]
	\centering
	\begin{tabular}{lllll} \hline	
	\rowcolor{verylightgray}
%	\begin{tabular}{|l|l|l|l|l|}\hline
		& v1   & v2   & v3  & v4  \\ \hline
		client1 & 1.1  &      & 1.2 &     \\ \hline
		client2 &      & 1.0  &     & 1.1 \\ \hline
		...     &   ...   &   ...   &  ...   &  ...   \\ \hline
		clientN & 1.02 & 1.12 & 1.2 & 2   \\ \hline
	\end{tabular}
	\caption{Dependency version matrix of a non-version library.}
	\label{tab:dependency-version-matrix}
\end{table}


%
%\begin{table}[h!]
%	\footnotesize
%	\centering
%%	\vspace{-.2cm}
%
%	\begin{tabular}{r p{11.0cm}} \hline	%p{0.25\linewidth}		
%		\rowcolor{verylightgray}
%		%		\toprule
%		\textbf{Score} & \textbf{Description} \\ \hline
%		%		\midrule		
%		0 & No results at all are returned \\ \hline
%		1 & The post is totally irrelevant \\ \hline %/The snippet contains help to the developer
%		2 & The post contains some hints but it is still out of context \\ \hline
%		3 & There are relevant suggestions but the key features are missing \\ \hline
%		4 & The post provides proper recommendations, together with its code snippets it can help developers solve their current task \\ \hline					
%		%		\midrule
%		%		& \textbf{Total} & \textbf{555} \\ %& \textbf{--,--}
%	\end{tabular}
%	\caption{Confidence Scores.}
%%	\vspace{-.3cm}
%	\label{tab:Scores}
%\end{table}



\begin{table}[h!]
	\centering
%	\begin{tabular}{|l|l|l|}
	\begin{tabular}{rrr} \hline	
		\rowcolor{verylightgray}
		& v2   & v4 \\ \hline
		client2 & 1.0  & 1.1  \\ \hline
		client3 & 2.12 & 3.01 \\ \hline
		...     &      &      \\ \hline
		clientN & 1.12 & 2    \\ \hline
	\end{tabular}
	\caption{Migrated client pairs of two specific library versions, \ie~v2 and v4.}
	\label{tab:client-pairs}
\end{table}

\aethereal includes various facilities that enable one to download and analyze static Maven artifacts. For instance, artifacts are manipulated as M3 models~\cite{7070485} which are automatically extracted from Java jar file with Rascal~\cite{5279910} to perform static analysis on the source or binary code. \aethereal supports the identification of clients that deal with the migration of library breaking changes.

\maracas is a framework developed by the CWI team to support automatic migration of client code according to changes in APIs. The delta, \ie~ changes that occur between two specific versions of the same library, and client detection model which identifies the parts of client code affected by the API evolution and must thus be migrated, are the key ingredients to tackle the API migration challenges. In this context, the \maracas framework gets through those steps and it is used in conjunction with \aethereal to identify deltas and detections over mined CPDMGs. Interested readers are kindly referred to Deliverable D2.8 ``API Analysis Components'' for more details on \maracas.


%Aethereal is a extensible tool that computes the 
%Aethereal is tools that builds CPMDG. This tools is developed by

\subsubsection{Analysis Results}\label{sec:aethereal-result}
In this section, we report the result of our mining studies. It is our firm belief that \Ad works more effectively given that more migration samples are available for recommendation. 

CPMDGs have been computed over 10 popular Maven dependencies. Table~\ref{tab:CPDMDG-report} gives a summary of the analyzed CPMDG: The columns \code{\#clients} and \code{\#versions} count the total number of clients that use any version of the library and the number of library version, respectively. As reported in Table~\ref{tab:dependency-version-matrix} \aethereal provides a dependency version matrix for each input library, then the \code{matrix density} column reports the number of non-empty cells over the total number of dependency version matrix cells. This value gives an intuition about how the clients have a proclivity for updating the library among the versions. The other columns report statical data of clients, \ie~average, min, max and the most used version. \code{org.sonarsource.sonarqube:sonar-plugin-api} library was included in the study to effectively support the FrondEndArt use case. 

In our study, migration samples are mined between two specific versions of the library. Clients update library in spontaneous ways, \eg~they change the library every update, they change the library version when a major version is released, or they never update the library. Migration client pairs analysis are presented in Table~\ref{tab:migration-report}. 
Tables~\ref{tab:gson-delta} and \ref{tab:guava-delta} report the delta changes computed by \maracas. In particular, Table~\ref{tab:gson-delta} summarizes the delta that occurs between two versions of \code{gson}, \ie~2.3.1 and 2.8.0, whereas the changes between guava 18 and guava 19 are shown in Table~\ref{tab:guava-delta}. Each delta change is related to a different element, \ie~Classes, methods and files, and different type of change, \ie~Method parameters, Static modifiers, Class/Interface implementation, Access modifiers, Abstract modifiers, etc. It is worth noting that the number of migration samples strongly depends on the distance between the targeting library version. 
In our study, detection models have been computed between two particular versions of a library and all initial client of clients pairs to detect which parts of client code are affected by the API evolution and thus must be migrated. An excerpt of clients detection is reported in Table~\ref{tab:guava-detections}. %In particular, 58 clients need to be migrated over 584 client pairs (see the first row of Table~\ref{tab:migration-report}).

% (\aethereal define the client pairs set)
%%MARACAS AND DELTA INTRODUCTION


\begin{landscape}
	
	\begin{table*}[h!]
		\vspace{2.0cm}
		\centering
		\begin{threeparttable}		
		\scriptsize
		\begin{tabular}{llllllllll} \hline	
		\rowcolor{verylightgray}
%		\begin{tabular}{|l|l|l|l|l|l|l|l|l|}\hline

			\textbf{id} &\textbf{Library}                                      & \textbf{\# clients} & \textbf{\# versions} & \textbf{matrix density} & \textbf{CPL (avg)}\tnote{*} & \textbf{CPL (min)}\tnote{*} & \textbf{CPL (max)}\tnote{*} & \textbf{MUV}\tnote{**} \\ \hline
			
			1& com.google.code.gson:gson                    & 43,727     & 35         & 0.029          & 1249.51                   & 0                         & 9979                      & 2.3.1             \\ \hline
		
			2& org.springframework.data:spring-data-jpa     & 1,298      & 83         & 0.012          & 14.0                      & 0                         & 94                        & 1.7.1.RELEASE     \\ \hline
		
			3& org.springframework.data:spring-data-mongodb & 5,840      & 84         & 0.011          & 69,53                     &           1                &        2388                   &          1.10.7.RELEASE         \\ \hline
			
			4& 	org.apache.common:commons-collections4                                      &  11,114     &    3       &       0.33         &    3704.66                       &           74                &      9392                     &      4.1             \\ \hline
			
			5& com.google.guava:guava                                    &     1,063,016  &    90       &    0.011            &           1182.7                &     0                      &        21753                   &        18.0           \\ \hline
			
			6& org.springframework:spring-core                             &      29,779 &   153       &     0.007           &       195.55                    &      0                     &            1384               &     3.0.5.RELEASE              \\ \hline
				
			7&joda-time:joda-time                                    &    52,003   &  38         &      0.026          &        1369.34                   &            0               &            9595               &       2.9.9            \\ \hline

			8& commons-cli:commons-cli                                   &  13,152     &      10     &        0.100        &             1315.2              &     1                     &      5376                     &      1.2            \\	\hline			
	
			9 & commons-io:commons-io                                   &  84,675     &      25     &        0.040        &             3392.08             &     0                     &      5376                     &      1.2            \\	\hline			
			
			10 & com.fasterxml.jackson.core:jackson-databind                                  &  73,870     &      121     &        0.008        &             611.22             &     0                    &      4542                     &      2.7.4            \\ \hline
			
			11	& org.sonarsource.sonarqube:sonar-plugin-api                                    &  365     &      60     &        0.017        &             6.08              &     0                      &      38                     &      5.6             \\ \hline
		\end{tabular}
	\begin{tablenotes}
		\small
		\item [*] Clients per library
		\item [**] Most used version
	\end{tablenotes}
	\end{threeparttable}
		\caption{Summary on CPMDG.}
		\label{tab:CPDMDG-report}
	\end{table*}

\begin{table}[h!]
	\centering	
	\scriptsize
%	\begin{tabular}{|l|l|l|l|p{1.2cm}|p{1.2cm}|l|p{2.0cm}|l|}\hline
	\begin{tabular}{llllllllll} \hline	
	\rowcolor{verylightgray}
		&\textbf{Library}                & \textbf{v1}   & \textbf{v2}   & \textbf{\# client pairs} &\textbf{ \# clients V1} & \textbf{\# clients V2} &\textbf{ \% migrated client}& \textbf{Major}  \\ \hline
		
		1 & com.google.guava:guava & 18.0 & 19.0 & 584            & 21753        & 19335        & 2         & Yes     \\ \hline		
		2 & com.google.code.gson:gson & 2.3.1 & 2.8.0 & 58            & 9979        & 2992        & 0.5        & Yes      \\ \hline
		3 & com.google.code.gson:gson & 2.8.0 & 2.8.2 & 129            & 2992        & 1972        & 4.31       & No      \\ \hline				
		4 & org.springframework:spring-core & 4.3.17.RELEASE & 4.3.18.RELEASE & 301            & 819        & 327        & 36.75	    & No          \\ \hline
		5 & org.springframework:spring-core &3.0.5.RELEASE & 4.3.8.RELEASE & 18            & 1384        & 1130        & 0.57	      & Yes        \\ \hline			
		6 & org.sonarsource.sonarqube:sonar-plugin-api:jar & 5.6 & 6.3 & 6            & 38        & 9        & 15.78     & Yes        \\ \hline
	\end{tabular}
 	\caption{Migration report.}
 	\label{tab:migration-report}	
\end{table}

\end{landscape}


\begin{table}[]
	\centering
	\footnotesize
	\begin{tabular}{ll} \hline	
		\rowcolor{verylightgray}
		\textbf{Change type}                          & \textbf{\# changes} \\ \hline
		Method parameters changed              & 1              \\
		Static modifiers changed               & 3              \\
		Class/Interface implementation changed & 3              \\
		Access modifiers changed               & 14             \\
		Abstract modifiers changed             & 0              \\
		Removed elements                       & 35             \\
		Added elements                         & 97             \\
		Renamed elements                       & 1              \\
		Final modifiers changed                & 1              \\
		Deprecated elements                    & 0              \\
		Moved elements                         & 109            \\
		Field and method types changed         & 1              \\
		Class extension changed                & 2             \\ \hline
		\textbf{Total} & \textbf{267} \\ \hline
	\end{tabular}
	\caption{Delta changes from \code{gson:2.3.1} to \code{gson:2.8.0}.}
	\label{tab:gson-delta}
\end{table}

\begin{table}[]
	\centering
	\footnotesize
	\begin{tabular}{ll} \hline	
		\rowcolor{verylightgray}
		\textbf{Change type}                                   & \textbf{\# changes} \\ \hline
		Method parameters changed              & 0     \\
		Static modifiers changed               & 0     \\
		Class/Interface implementation changed & 1     \\
		Access modifiers changed               & 1     \\
		Abstract modifiers changed             & 3     \\
		Removed elements                       & 3     \\
		Added elements                         & 5     \\
		Renamed elements                       & 0     \\
		Final modifiers changed                & 1     \\
		Deprecated elements                    & 12    \\
		Moved elements                         & 2     \\
		Field and method types changed         & 0     \\
		Class extension changed                & 3     \\ \hline
		\textbf{Total}                                  & \textbf{31}   \\ \hline
	\end{tabular}
	\caption{Delta changes from \code{guava:18.0} to \code{guava:19.0}.}
	\label{tab:guava-delta}
\end{table}

\begin{table}[]
	\centering
	\scriptsize
%	\begin{tabular}{|l|p{2.0cm}|p{2.0cm}|l|l|p{2.0cm}|}\hline
	\begin{tabular}{llllll} \hline
		\rowcolor{verylightgray}
		& \multicolumn{5}{c|}{\textbf{Client detection types}}                                          \\ \hline
		\textbf{Client}                       & \textbf{ABSTRACT MODIFIER} & \textbf{ACCESS MODIFIER }& \textbf{DEPRECATED} & \textbf{EXTENDS} & \textbf{FINAL MODIFIER} \\ \hline
		cassandra-driver-core-2.1.6  & 0                  & 0                & 11         & 48      & 0               \\ \hline
		async-datastore-client-2.1.0 & 0                  & 0                & 22         & 34      & 0               \\ \hline
		futures-extra-2.6.1          & 0                  & 0                & 3          & 44      & 0               \\ \hline
		helios-client-0.9.25         & 0                  & 0                & 16         & 29      & 0               \\ \hline
		herdcache-1.0.31             & 0                  & 0                & 0          & 35      & 0               \\ \hline
		calcite-core-1.11.0          & 18                 & 0                & 0          & 0       & 17              \\ \hline
		gfc-guava\_2.10-0.1.4        & 0                  & 0                & 8          & 20      & 0               \\ \hline
		gfc-guava\_2.11-0.1.3        & 0                  & 0                & 8          & 20      & 0               \\ \hline
		folsom-0.7.1                 & 0                  & 0                & 3          & 22      & 0               \\ \hline
		bigtable-client-core-0.2.1   & 0                  & 0                & 2          & 20      & 0               \\ \hline
		gax-0.12.0                   & 0                  & 0                & 0          & 18      & 0               \\ \hline
	\end{tabular}
	\caption{An excerpt of client detections over 584 clients migrating from \code{guava 18.0} to \code{guava 19.0}.}
	\label{tab:guava-detections}
\end{table}

==> src/mbn.tex <==

In recent years, \GH has been at the forefront of platforms for storing, 
analyzing and maintaining the community of OSS projects. To foster the 
popularity and reachability of their repositories, \GH users make daily 
usage of the star voting system as well as forking 
\cite{borges_whats_2018,Jiang:2017:WDF:3042021.3042043}. These 
features allow for increasing the popularity of a certain project, even though the 
search phase has to cope with a huge number of items. To simplify this task, 
\GH has introduced in 2017 the concept of \emph{topics}, a list of tags 
aiming to describe a project in a succinct way. Immediately after the 
availability of the topics concept, the 
platform introduced Repo-Topix 
\cite{ganesan_topic_2017} to assist developers when creating new projects and 
thus, they have to identify representative topics. 

%As discussed in \cite{10.1145/3383219.3383227}, 
Though Repo-Topix is 
already in place, there are rooms for improvements, \eg in terms of the 
coverage of the recommended topics, and of the underpinning analysis 
techniques. To this end, we proposed an 
approach~\cite{10.1145/3383219.3383227} based on a Multinomial Naive Bayesian network technique to 
automatically recommend topics given the \RM file(s) of an 
input repository. 
%
%%% IT SEEMS THESE ARE MORE CHALLENGES TO BE MOVED LATER IN THE PAPER
%As we are in the machine learning (ML) domain, 
%there are several issues to face during the development, especially ones that 
%concern the definition of the training set. On one hand, the model suffers 
%from 
%performance degradation with a large set of possible outcomes. On the other 
%hand, reducing 
%the set of retrieved items affects the effectiveness of the 
%recommendation. We 
%manage this trade-off by limit our analysis to a curated list of 
%topics, namely 
%\emph{featured} topics. According to \GH statistics, this list 
%represents the 
%most popular topic spread over the entire community \cite{featured}. 
%Another 
%challenge in the ML domain is the balancing of the dataset. 
%Considering the 
%supervised approaches, in which the model knows ex-ante the possible 
%outcome, a 
%training set can be balanced or unbalanced. The former indicates that 
%the 
%possible classes have the same number of samples. In the latter, the 
%samples 
%are spread in a not uniform fashion. Due to the Naive Bayesian 
%internal 
%construction, we used a balanced dataset of 134 featured topics to 
%mitigate the 
%mentioned issues. 
%
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.9\textwidth]{figs/MNBArch.png}
	\caption{Overview of the \bnetwork~approach~\cite{10.1145/3383219.3383227}.}
	\label{fig:mnb}
\end{figure}
%
The overall architecture of the approach is depicted in 
Fig.~\ref{fig:mnb}. First of all, we created the initial dataset by 
downloading the \RM files for each repository that are tagged with a featured 
topic\footnote{\url{https://github.com/topics}} in the \emph{\GH crawling} 
phase. To this end,  we exploited the \GH API 
offered by the PyGitHub library \cite{pygithub/pygithub_2019} to retrieve all the 
needed data. To deal with the authorization limit in the requests, we used the 
\GH query language to filter the repositories list using the following query:
\begin{equation}
Qf = "is:featured \; topic:t \; stars:100..80000 \; topics:>=2"
\end{equation}
taking into consideration \GH repositories having a number of stars between 100 
and 80,000, and 
tagged with at least two topics. The obtained \RM files are encoded by adopting 
the TF-IDF vectorizer class of the Scikit-learn 
library.\footnote{\url{http://scikit-learn.org}} The \emph{\RM encoding} phase is 
necessary to feed the network with features vector representing the entire 
content of a \RM file. Then, the training phase is enabled and the list of 
predicting topics is retrieved using the multinomial probability distribution 
embedded in the MNB network in the \emph{Topic prediction} phase. The approach 
relies on the strong assumption that each variable is conditionally independent, 
\ie no relationship holds among the elements of the population. Nevertheless, 
the model is successfully employed in different applications as the mentioned 
precondition rarely occur in practice. Once the initial list of topics had been 
retrieved in such a way, we employed the GuessLang external 
tool\footnote{\url{https://pypi.org/project/guesslang/}} to perform \emph{Language prediction}, \ie predicting topics related to programming 
languages. The rationale behind this choice is due to the MNB internal 
construction. In particular, predicting a language tag requires a deep analysis 
of the source code that goes beyond the model's capability. Thus, a reliable external library developed for this specific purpose has been used to predict 
language-related topics, \ie Java, Python, C. Finally, \emph{Topic aggregation} is conducted in which the predicting featured topics retrieved by 
the MNB network were combined with the ones discovered by GuessLang. As the 
model ranks the final outcomes using their probability, the last element of the list is substituted with the one delivered by GuessLang.  Furthermore, lightweight NLP techniques have been applied on the topics during the comparison, \ie stemming and dashes removal. The approach has been evaluated using the ten-fold cross validation technique considering only the featured topics of a testing project.
